An Efficient Framework for Computing Structure- And Semantics-Preserving Community in a Heterogeneous Multilayer Network

Multilayer networks or MLNs (also called multiplexes or network of networks) are being used extensively for modeling and analysis of data sets with multiple entity and feature types and associated relationships. Although the concept of community is widely-used for aggregate analysis, a structure- and semantics preserving definition for it is lacking for MLNs. Retention of original MLN structure and entity relationships is important for detailed drill-down analysis. In addition, efficient computation is also critical for large number of analysis. In this paper, we introduce a structure-preserving community definition for MLNs as well as a framework for its efficient computation using the decoupling approach. The proposed decoupling approach combines communities from individual layers to form a serial k-community for connected k layers in a MLN. We propose a new algorithm for pairing communities across layers and introduce several weight metrics for composing communities from two layers using participating community characteristics. In addition to the definition, our proposed approach has a number of desired characteristics. It: i) leverages extant single graph community detection algorithms, ii) introduces several weight metrics that are customized for the community concept, iii) is a new algorithm for pairing communities using bipartite graphs, and iv) experimentally validates the community computation and its efficiency on widely-used IMDb and DBLP data sets.

==> texFiles/ExtendedAbstract_Final.tex <==
\section*{Extended Abstract}

\textbf{Introduction and Topic.} In this paper we address the important problem of identifying communities in heterogeneous multilayer networks. While single layer networks are used to represent systems of interacting/interrelated entities, multilayer networks represent relations between multiple single layer networks. There exist two main types of multilayer networks (or multiplexes) \cite{BDA/SantraB17}. The first type is homogeneous multiplex, where the type of entity in each layer is same. An example would be different types of social networks between the same set of people, each layer representing a different type of social media like Facebook, LinkedIn etc. The second type is heterogeneous multiplex, where the type of entities in each layer may be different. An example would be a combination of a protein interaction network and drug interaction network, where the proteins in the top layer are connected to the relevant drugs in the bottom layer.

Community detection algorithms have been extensively studied for single layer networks, and there are also some algorithms for homogeneous networks ~\cite{dong2012clustering,li2008scalable,zhang2017modularity, ICCS/SantraBC17}. However, community detection algorithms for heterogeneous networks is relatively sparse, and even the definition of communities is not clear in this context. There is also a lack of flexibility in the current community detection algorithms for multilayer networks. Most community detection algorithms for multilayer networks consider the entire network as a whole. Thus if the user needs to compare between different subsets of layers or to add a new layer to a previously created multilayer network, then the entire communities have to be re-computed. This approach also fails to identify by how much a vertex contributes to inter-layer communities (i.e. communities within its own layer) and intra-layer communities (communities across layers).

To address this issue of flexibility we present a composition-based algorithm for finding communities in heterogeneous multilayer networks, that can (i) update communities rather re-computing them from scratch if the number of layers change and  (ii) clearly identify the contribution of the vertices in the inter-layer and the intra-layer communities.

\textbf{Key Concepts.} The main principle of our algorithm is to analyze the communities of the constituent networks separately, and then combine these results to produce the integrated results for the entire multilayer network or a subset of the layers, as needed. We define pair-wise combination as the operation by which a pair of constituent networks are combined. We define aggregation operation as the operation by which the analysis results, here community detection, of two constituent networks are combined. The goal of network composition is, given a pair-wise combination operation and analysis function, \textbf{to create an appropriate aggregation operation, such that the integrated results of constituent networks is the same as the result of the multilayer network formed by combining the network pairs.}

Network composition provides the following advantages that are not available in the current
method of analyzing the combined multilayer network.

\begin{itemize}
\item \textit{Uniform approach of analysis.} Currently, homogeneous and heterogeneous networks are
treated as separate types of networks.  When using network composition, users do not have to distinguish among network types except when combining the results. 

\item \textit{Scalability to large datasets.} Network composition allows us to analyze constituent networks
in parallel, thus making the analysis more scalable. We can further improve the scalability by analyzing each constituent network using parallel algorithms developed for monoplexes. 

\item \textit{Leveraging algorithms of single networks.} By using network composition, we can leverage
the rich set of analysis algorithms for monoplexes, including approximation algorithms and methods for updating dynamic networks to the multilayer domain.

\item \textit{Re-usability of results.} By applying network composition, we can reuse the results of the constituent networks. This significantly reduces the analysis time when the same constituent network is present in different multilayer networks. This allows users to easily experiment with different combinations and interactions of the constituent networks.

\end{itemize}


\textbf{Methods.} Formally, we define $G_1$ and $G_2$ be a pair of networks.  Let $L$ be a bipartite graph consisting of edges connecting a vertex of $G_1$ to one or more vertices of $G_2$.  Let the analysis function be $F$, the combination operation be $\theta$, and the aggregation operation be $\phi$. Our goal is given $G_1, G_2, L, F, \theta$, find $\phi$, such that  $F(\theta(G_1, G_2, L))= \phi(F(G_1), F(G_2), \theta, L) $.

In the case of \textbf{heterogeneous} networks, the edges in $L$ represent how the vertices in $G_1$ and $G_2$ interact with each other. In this case $L$ is an important part of network combination (a \textbf{bi-partite graph} between two layers), and should be included in designing the aggregation operation. 
 
To find communities in heterogeneous multilayer networks, we present a method, which we term as \textit{community-induced bipartite graphs}. We first detect the communities for each layer. Once the communities are detected, then using the communities and inter-layer edges from two layers a \textit{bipartite graph} is created, such that each community becomes a \textit{meta node} and the inter-layer edges between the communities from each layer become \textit{meta edges} (which can be weighted). In order to compute the \textit{optimal sets of communities that have maximum interaction among themselves}, we have proposed network flow-based composition techniques.  

\textbf{Focus of This Paper.} In this paper, we focus on demonstrating that composition based community detection can lead to more efficient and more meaningful communities in multilayer networks. To this end, we will particularly focus on multilayer networks created from IMDB dataset \cite{data/type2/IMDb}. The 2-layer IMDB multiplex has one layer for actors connected by an edge if they have acted together in some movie and another layer for directors connected based on directing similar movie genres. The inter-layer edge represents the who-directs-whom relationship. Experiments conducted as a part of this paper have focused on the following aspects

\begin{itemize}
\item Comparing the diverse types of communities obtained from a multiplex with respect to single graph (monoplex) that does not distinguish between the types of entities (i.e., actors and directors.)
\item Evaluating the quality of the heterogeneous communities obtained and the performance of the proposed technique.
\item Additional layers based on movie ratings, Oscars won etc. have been used to signify the flexibility of the proposed approach in analyzing the IMDB multiplex from different aspects to produce insights like dominant genre evolution, nature of actor and director communities, prominent co-actor groups in the top-rated set of movies and so on.
\end{itemize}

\textbf{Expected Results.} We will compare our results with the standard approach for community detection on multilayer networks, and demonstrate that our composition-based approach can provide more information about how the vertices contribute to their respective communities. We will also show that our approach is faster, in the case where the layers comprising the multilayer network change.

\textbf{Conclusion.} In this paper, we present a composition based approach for identifying communities in heterogeneous multilayer networks using network flow techniques on bipartite graphs. We use the IMDB dataset as a case study for  highlighting the benefits of our approach, namely more information about the composition of communities within and across layers and faster recomputing of communities when the layers change.

==> texFiles/ExtendedAbstract_SC.tex <==
%Submit an extended abstract (approx. 1000 words) no later than October 01, 2018. The proposal should include: Topic, Key concepts, Methods, Expected Results and Conclusions. Please ensure that you include your full name and email contact details.  

\section{Topic}
\label{sec:topic}
In this paper we address an important topic in big data analytics, that of finding communities in multilayer networks. Multilayer networks are used to represent datasets with different types of features. For example, social networks


Big data analytics is increasingly used to ascertain known trends as well as infer new potentially counter-intuitive inferences. %These analytics are useful from a business perspective as well. Many approaches are being developed and used depending upon the dataset, its characteristics, and what needs to be inferred. 
In this paper, we address a category of datasets that is characterized by features of different types of entities. %For example, a movie data set consisting of directors, actors, and genre that may be relevant to both actors and directors. Actors acting together or in the same genre may be needed for certain analysis. 
Such data sets with multiple types of entities can be modeled using  heterogeneous multilayer networks. Social networks fall into this category with people as entities and features corresponding to age, location, marital status, political views, communication preferences, etc.  %Other datasets (e.g., accident datasets) are also characterized by multiple features, such as weather, road condition, speed, light condition, for each accident \cite{Arxiv/santra2016scalable}. These data sets can be modeled using homogeneous multilayer networks. 
In this paper, we summarize the challenges associated with analyzing heterogeneous multilayer networks and present a novel algorithm for finding communities comprised of multiple layers of heterogenenous networks.
%A case study will be used to illustrate our approach.

\section{Key Concepts}
The key concept explored in this paper is that of a community in heterogeneous networks.

%\textbf{Community Detection in Monoplexes} (single graphs) involves identifying groups of vertices that are more connected to each other than to other vertices in the network. This objective is often translated into the problem of optimizing network parameters such as modularity ~\cite{Clauset2004} or conductance ~\cite{Leskovec08}. The combinatorial optimization problems for community detection are NP-complete ~\cite{Brandes03}.
%A large number of competitive approximation algorithms exist (see reviews in ~\cite{porter09, Fortunato2009, Xie2013}). 
%Algorithms for community detection have been developed for a wide range of inputs including directed ~\cite{Leicht08,Yang10}, weighted ~\cite{Berry2011}, and dynamic networks ~\cite{Bansal2011,porterchaos13}.  

\textbf{Community Detection in Multilayer Networks:} has been addressed mainly with respect to the \textbf{homogeneous} variant, where every layer has the same set of nodes and there are no inter-layer edges. It includes algorithms based on matrix factorization \cite{dong2012clustering, qi2012community}, pattern mining \cite{zeng2006coherent,silva2012mining},  cluster expansion philosophy \cite{li2008scalable}, Bayesian probabilistic models \cite{xu2012model} and regression \cite{cai2005mining}. Techniques for determining communities in temporal homogeneous multilayer networks using spectral optimization  of the modularity function based on the supra-adjacency representation have also been proposed \cite{zhang2017modularity,bazzi2016community}. Moreover, to study the combinations of different layers in the network some efficient approaches have been proposed where communities obtained from individual layers are combined to obtain communities in any Boolean operation based combined layer  multilayer network \cite{ICCS/SantraBC17,Arxiv/santra2016scalable}.

However, there \textbf{does not exist a consensus on the definition of communities for heterogeneous multilayer networks}. The presence of different sets of entities, inter- and intra-layer edges makes these tasks more challenging. Few existing works have proposed techniques for generating clusters of entities \cite{sun2009rankclus, sun2009ranking,melamed2014community}, but they have only considered the inter-layer links and not the network layers. Thus, the combined effect of intra- and inter-layer relationships have not been addressed which is the focus of this paper.

\section{Methods}
 The main principle of  network composition is to analyze the constituent networks separately, and then combine these results to produce the integrated results for the entire multilayer network or a subset of the layers. 

We define {\em pair-wise combination} as the operation by which a pair of constituent networks are combined. We define {\em aggregation operation} as the operation by which the analysis results of two constituent networks are combined. The goal of network composition is,  given a pair-wise combination operation and analysis function, {\bf to create an appropriate aggregation operation, such that the integrated results of constituent networks is the same as the result of the multilayer network formed by combining the network pairs.}

In a homogeneous multilayer network, 
%the relationship or similarity among a given set of people will vary with features under consideration. That is, 
each layer has the same nodes, BUT their edge connectivity will vary according to the feature value distribution. For example, actors who worked together in a movie could be represented in one layer and actors who have worked in the same genre could be represented in another layer. A community in a graph translates to a group of nodes that are more connected to each other than to other nodes in the graph. To detect communities, we use widely-used packages, Infomap\cite{InfoMap2014} or Louvain~\cite{}. 

If one wants to identify groups of actors who have worked together and in the same genre, the communities from two layers need to be composed to obtain the same answer that would have obtained if we had a monoplex representation. This requires composition of communities in a loss-less manner. Our work has proposed loss-less approaches to community detection for homogeneous multiplexes for Boolean operations (AND, OR and NOT).

\textbf{Community Detection for \textit{AND}-Compositions:} One way to answer the above question is to first generate the combined graph corresponding to the \textit{AND}-composition and then detect the communities (termed \textit{NA\"{I}VE-COMM} method). This entails, for a given dataset with $k$ attributes, generating O($2^{k}-1$), individual and \textit{AND}-composed graphs, and computing communities in each of them. 

In contrast, our approach (termed \textit{EFF-COMM}) generates only \textit{k} graphs (for \textit{k} layers) and composes the communities computed for each layer~\cite{ICCS/SantraBC17}. It can be shown analytically that both computationally and storage-wise, \textit{EFF-COMM} is more efficient. The requirement to apply \textit{EFF-COMM}, is that the communities of the individual layer must be \textit{self-preserving} in nature. Even if they are not, by using a different approach (edge intersection~\cite{}  instead of node intersection~\cite{}), we can obtain the resulting community.

\subsection{\textbf{Focus of This Paper}}

Formally, let $G_1$ and $G_2$ be a pair of networks.  Let $L$ be a bipartite graph consisting of edges connecting a vertex of $G_1$ to one or more vertices of $G_2$.  Let the analysis function be $F$, the combination operation be $\theta$, and the aggregation operation be $\phi$. Our goal is given $G_1, G_2, L, F, \theta$, find $\phi$, such that 
$F(\theta(G_1, G_2, L))= \phi(F(G_1), F(G_2), \theta, L) $.

If the network pairs are \textbf{homogeneous} to each other, then $L$ simply maps a vertex in $G_1$ to its corresponding vertex in $G_2$, and can thus be ignored for the combination operation.  However, for \textbf{heterogeneous} networks, the edges in $L$ represent how the vertices in $G_1$ and $G_2$ interact with each other. In this case $L$ is an important part of network combination (a \textbf{bi-partite graph} between two layers), and should be included in designing the aggregation operation. 

We have classified the common combination operations appearing in the literature on multilayer analysis, into these four categories~\footnote{The names have been defined by us due to the absence of any nomenclature regarding the combination operations.}. We will develop aggregation operation for each pair of analysis function and combination operations. Out of these four combination operations, projection-based is the only one that is not commutative and has to be defined on a pair of networks. The other operations can be defined on a set of networks and are commutative. The following are applicable to heterogeneous networks.

\begin{itemize}
\item \textbf{Community-induced bipartite graphs} Here communities are detected for each layer as in the case of a homogeneous approach. Once the communities are detected, a bipartite graph is created using each community as a meta node and representing the edges between communities from two layers as edges (can be weighted). These bipartite graphs are analyzed using flow-based approaches.

\item {\bf Type-independent Combination} Here the types of the vertices in $G_1$ and $G_2$ are ignored and all vertices are treated as of a single type. A combined graph is formed by the union of the vertices in $G_1$ and $G_2$ and the union of the edges in  $G_1$, $G_2$ and $L$. This combined graph is analyzed.

\item {\bf Projection-based Combination} Here a new network $\bar{G_1}$ is created, where two vertices are connected if they have common neighbors in the bipartite graph $L$.  Thus $\bar{G_1}$ represents the inter-relation of $G_1$ with respect to $G_2$. Since $G_1$ and $ \bar{G_1}$ form a homogeneous pair, they can then be combined using the Boolean or linear combination.
\end{itemize}

This paper focuses on composing communities from two or more layers using \textbf{community-induced bipartite graphs} between two layers. We propose approaches for composing two or more layers using computations on multiple bipartite graphs induced by the composition. We will use the IMDb data set to show complex analysis as well as validate our approaches and compare the results with ground truth where available.

\section{Expected Results}
The expected results of this work are:

\begin{itemize}
\item Contrast the approaches needed for homogeneous multilayer network analysis. They are not the same. Composition of heterogeneous layers is more challenging and has multiple options that may be relevant to different types of analysis
\item Bipartite graph-based approaches for composing heterogeneous multilayer networks and their flexibility
\item Mapping analysis questions to heterogeneous multilayer networks
\end{itemize}

\section{Conclusions}
In this paper, we have presented the challenges in analyzing a data set representation using heterogeneous multilayer networks. We have related the analysis to the benefits of this representation as well as the composition alternatives useful for doing the analysis. A real-world data set used as a case study for illustrating the approach, analysis, and results.

==> texFiles/Metric_back.tex <==
\section{k-Community Detection in Heterogeneous MLNs}
\label{sec:hemln-community}

In the previous section, based on the analysis requirements it has been highlighted how datasets need to be modeled as HoMLN and/or HeMLN. Further, it can be observed that the analysis requires the detection of communities. In case of HoMLN (Accident and Facebook), decoupling-based strategies have been proposed to compose communities based on different features \cite{BDA/SantraB17,ICCS/SantraBC17}. The problem arises when we wish to find \textit{communities involving multiple types of entities}. For instance, for the heterogeneous IMDB multilayer network shown in Figure \ref{fig:HeMLN-examples} (b), \textit{what will define a community of actors and directors?}. Clearly, multiple relationships exist in such a group like co-acting, similar genres and who-directs-whom. An analysis query requirement may want to give \textit{difference preference levels} to each one of them. For example, one may be interested in the groups where the actors and directors interact the most (Query 4a), while some other query may require the most sought after co-actors to be interacting with the most versatile directors (Query 4c). %Traditional approaches of a) treating the heterogeneous network as a whole by removing type information and applying community detection or b). projecting one layer onto another and then finding communities, will give results that  either hide the effect of different entity types and/or different intra- or inter-layer relationship combinations leading to loss of or misleading information.
The homogeneous network community composition based techniques will not be applicable as each layer has different sets of entities.
%It is important to note that this formulation of communities preserves entity and feature types as compared to other alternatives proposed in the literature.
Moreover, existing approaches that either i)  combine (or aggregate) all the layers, ignore types and apply single graph community detection algorithms or ii) project a layer on to a connected layer as a means of aggregating the two layers and apply single graph community detection, again ignoring entity types will give results that  either hide the effect of different entity types and/or different intra- or inter-layer relationship combinations leading to loss of or misleading information.
The problem escalates when new entities and/or relationships get involved like movies having similar IMDB ratings/gross collections/language, production houses, country of release, actor nationality and so on, as the scope of queries increases. Therefore, there is a \textit{need for an efficient approach that can detect the community of different sets of entities where the entity and relationship type is preserved based on the requirements of the analysis query}.

%In advertising, the agencies look to maximize the reach of an advertisement in minimum amount of time. Thus, a group of Facebook (or any other social media) friends who are well-connected based on the features of the ad become a possible target audience. Similarly, for installing effective accident prevention measures it is important to find out accident prone regions with respect to the poor lighting conditions, bad weather and so on. Some other similar interesting analysis from other domains include - group of well-connected cities by different airlines, strongly connected group of co-actors working in particular movie genres, similar group of research collaborations publishing in specific conferences and so on. Such queries require the finding out of entities that are more similar to each other as compared to other entities based on a set of features. In graph terminology, this corresponds to detecting \textit{communities of nodes that are well-connected through edges with each other as compared to other nodes in the graph}. 

%However, all these cases take into account a \textit{single type of entity} like Facebook users, accident locations, authors, actors or cities. Ample work has been done to compose communities based on different features by modeling such complex interaction networks as homogeneous multilayer networks \cite{BDA/SantraB17,ICCS/SantraBC17}. The problem arises when we wish to find \textit{communities involving multiple types of entities}. For instance, for the heterogeneous IMDB multilayer network shown in Figure \ref{fig:HeMLN-examples} (b), \textit{what will define a community of actors and directors?}. Clearly, multiple relationships exist in such a group like co-acting, similar genres and who-directs-whom. An analysis query requirement may want to give \textit{difference preference levels} to each one of them. For example, one may be interested in the groups where the actors and directors interact the most, while some other query may require the most sought after co-actors to be interacting with the most versatile directors. Traditional approaches of treating the entire heterogeneous network as a whole to detect communities will give results that hide the effect of different relationship combinations leading to loss of or misleading information. On the other hand, homogeneous network composition based techniques will not be applicable as each layer has different sets of entities. The problem escalates when new entities and/or relationships get involved like movies having similar IMDB ratings/gross collections/language, production houses, country of release, actor nationality and so on, as the scope of queries increases. Therefore, there is a \textit{need for an approach that can detect the strong groups of different types of entities based on the requirements of the analysis query}. 

In this section, we dwell into the problem of detecting communities for two layers, say $G_i$ and $G_j$ that are connected based on the bipartite graph, $X_{i,j}$. With respect to the entities from these two layers, there are three types of interactions a) interaction among the entities in layer $G_i$, b) interaction among the entities in layer $G_j$ and c). interaction between the entity sets from $G_i$ and $G_j$. %In order to obtain strongly knit groups of 2 different entities, i.e. 2-communities these three interactions need to be maximized among the group members. Applying the existing community detection techniques by removing the node and edge type information and considering the multiplex as a whole will
Informally, a strongly knit group of 2 different entities, i.e. 2-community, that \textit{preserves the entity types and relationships among them}, must be such that all \textit{these three interactions are maximized among its members, separately}. Maximizing the interactions among entities of same type (as in a) and c)) translates to the layer-wise communities (in layers $G_i$ and $G_j$). Further, maximizing the interactions between entities from two different sets translates to an optimal pairing of communities from two layers. However, this pairing of communities depends on the analysis requirements that lead to \textit{inter-layer interpretations} like maximizing a specific \textit{proportion} of interaction, maximizing interaction among community members \textit{satisfying a graph property} and so on. Based on this discussion, the formal definition for a 2-community has been given below,

\noindent\textbf{2-Community:} \textit{For a chosen inter-layer interpretation, $\phi$, $C_{i,j}^r(V_i^r, E_i^r, V_j^r, E_j^r, E_{i,j})$ is a 2-community with respect to $G_i$ and $G_j$, if a). $C_i^r(V_i^r, E_i^r)$ is a community in $G_i$, b). $C_j^r(V_j^r, E_j^r)$ is a community in $G_j$ and c). maximizing $\phi$ leads to the pairing of $C_i^r$ and $C_j^r$}.

As discussed, an optimal matching of the layer-wise communities is required such that the chosen interpretation of the inter-layer interaction is maximized. In bipartite graphs, maximum flow-based matching algorithms like Ford-Fulkerson give a set of pairings such that the overall flow across the network is maximized \cite{}. Thus, by generating a \textit{meta-bipartite graph} where the layer-wise communities become two sets of meta nodes which are connected by a meta edge if any of the members of meta nodes from different sets are connected in the actual multiplex, this problem can be mapped to a network flow problem. Therefore, based on the inter-layer interpretation, $\phi$, derived from the analysis requirements, if appropriate weights are specified on the inter-layer meta edges such that the \textit{optimal matching of communities is obtained that will be combined to form the 2-communities}. 

\begin{algorithm}
\caption{Algorithm for 2-Community Detection}
\label{algo:2-community}
\begin{algorithmic}[1]
   \REQUIRE $C_i$: Set of Communities from $G_i$, $C_j$: Set of Communities from $G_j$ , $X_{i,j}$, $\phi$, $C_{i,j}$ = $\emptyset$

Generate the Meta-bipartite graph, $X'_{i,j}(V'_i, V'_j, L'_{i,j})$
   \STATE $V'_i$ = $\emptyset$, $V'_j$ = $\emptyset$, $L'_{i,j}$ = $\emptyset$
   \FORALL {$C_i^m \in C_i$}
       \STATE $V'_{i} \gets V'_{i} \cup u'_m$
   \ENDFOR
   
    \FORALL {$C_j^m \in C_j$}
       \STATE $V'_{j} \gets V'_{j} \cup v'_m$
   \ENDFOR

    \FORALL {$u'_m \in V'_i$}
    	    \FORALL {$v'_n \in V'_j$}
            \IF {$\exists$a,b: ($u_a$, $v_b$) $\in$ $X_{i,j}$, where, $u_a$ $\in$ $C_i^m$ and $v_b$ $\in$ $C_j^n$}
       \STATE $X'_{i,j} \gets X'_{i,j} \cup (u'_m, v'_n)$            \ENDIF
            \ENDFOR

   \ENDFOR
    \FORALL {$(u'_m, v'_n) \in X'_{i,j}$}
       \STATE Assign weight, $w(u'_m, v'_n)$, based on $\phi$
   \ENDFOR
   
   \STATE Apply Maximal Matching Algorithm to get 2-community set, $C_{i,j}$
\begin{comment}


   \FORALL {$u_m^{k} \in V_{k}$}
       \STATE $V_{k'} \gets V_{k'} \cup u_m^{k'}$
   \ENDFOR

   \FORALL {$ u_m^{k'}, u_n^{k'} \in V_{k'}, m > n$}
       \IF {$(u_m^{k}, u_n^{k}) \notin E_{k}$}
           \STATE $E_{k'} \gets E_{k'} \cup (u_m^{k'}, u_n^{k'})$
       \ENDIF
   \ENDFOR
\end{comment}
\end{algorithmic}
\end{algorithm}

Algorithm \ref{algo:2-community} gives the process to detect 2-communities for layers, $G_i$ and $G_j$ for the chosen inter-layer interpretation, $\phi$.
A decoupling-based approach is followed for detecting communities for 2 layers, where the layer-wise communities are generated only once and combined as required. Based on the analysis requirements, a meta-bipartite graph, $X'_{i,j}(V'_i, V'_j, L'_{i,j})$, is formed using the communities from $G_i$ and $G_j$ that are treated as meta nodes for the two sets ($V'_i, V'_j$) who are connected by inter-layer meta edges ($L'_{i,j}$) such that any of the member pairs from the communities is connected. Weights are specified on the inter-layer meta edges based on the inter-layer interpretation, $\phi$. Network flow algorithm is applied on this graph to obtain the community pairings that are combined to form the 2-community. Next we will discuss the various interpretations of inter-layer interaction maximization.

\subsection{Inter-layer Interaction Interpretation ($\phi$) Classes}
Based on the requirements of the analysis, the interaction between the entities of different types can have multiple interpretations. In this paper, broadly we have discussed three classes of interpretations based on aggregation of interaction (Sec \ref{sec:m1}), density of interacting communities (Sec \ref{sec:m2}) and participating hubs in the interaction (Sec \ref{sec:m3}). In this section, we discuss how these different interpretations will effect the weights of the inter-layer meta edges in the meta-bipartite graph such that the maximal flow based matching algorithms give the community pairings with desired characteristics. Moreover, we will show how the requirements of the queries listed in Section \ref{sec:modeling} can be mapped on one of these. 

\subsubsection{Aggregate Interaction ($\phi_A$)}
\label{sec:m1}
Certain queries will need the detection of groups where apart from strong interaction among the same type of entities, \textit{maximum interaction exists among entities from different sets}. Therefore, in this case, weight of the inter-layer meta edges should reflect number of interactions that exist between the members of every community pair from two layers.  Formally,
\\

\noindent \boldsymbol{$\phi_A$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that
\begin{itemize}
\item maximum number of member pairs from paired communities are connected, then
\end{itemize}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight, }

\textit{\centerline{w(u', v') =  $|L_{i,j}^{m,n}|$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$
}
\\

Query 3a. from DBLP and query 4a. from IMDB fall under this class where maximum number of author-conference connections and actor-director connections need to be considered for answering the query.

\subsubsection{Dense Community Interaction ($\phi_D$)}
\label{sec:m2}
Another class of queries will require the larger fraction of the members belonging to the \textit{dense entity groups} from both the layers to interact. In contrast to $\phi_A$, here the layer-wise community characteristics will play a role in the matching. Apart from that, instead of \textit{number} of interactions, this interpretation takes into account the \textit{fraction} of total member pairs from communities that are interacting. Clearly, \textit{higher the densities and larger the fraction, stronger is the interaction among same and different types of entities, respectively}. Thus, the directly proportional behavior of these parameter shows that they must be multiplied to represent the inter-layer meta edge weight for this interpretation. The domain of this weight will be $(0,1]$ and it will be 1 when both the communities are cliques and all the members from both layers interact with each other. Formally,
\\

\noindent \boldsymbol{$\phi_D$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that,
\begin{enumerate}[label=\roman*.]
\item dense communities are paired and,
\item larger fraction of member pairs from paired communities are connected, then
\end{enumerate}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight,}

\textit{\centerline{ w(u', v') =  $\frac{2*|E_i^m|}{|V_i^m|*(|V_i^m|-1)}$ * $\frac{|L_{i,j}^{m,n}|}{|V_i^m|*|V_i^n|}$*$\frac{2*|E_j^n|}{|V_j^n|*(|V_j^n|-1)}$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$.
}
\\

In query 3b. from DBLP, the largest research domains will correspond to the densest communities from conference layer and tight co-author groups will be the dense communities from author layer. Thus, along with the requirement to check whether \textit{most of the members} of co-author publish in similar conferences, this query complies with the specifications of $\phi_D$. Similarly,  query 4b from IMDB also gets mapped to $\phi_D$, as tight co-actor groups and most popular genres correspond to communities in actor and director, respectively and fraction of total number of who-directs-whom interactions needs to be maximized.



\subsubsection{Hub Interaction ($\phi_H$)}
\label{sec:m3}
The third class of queries that we have considered will require that apart from a \textit{large fraction of the interacting member pairs}, the \textit{most central entities} from each group also interact across layers. Thus, here the inter-layer interaction takes into consideration the number of community-wise hubs that participate in the interaction. High centrality nodes (or hubs) can be defined based on metrics like degree centrality (vertex degree), closeness centrality (mean distance of the vertex from other vertices), betweenness centrality (fraction of shortest paths passing through the vertex), and eigenvector centrality. In this paper, we have used degree centrality as the metric. Similar to $\phi_D$, as \textit{higher the ratio of participating hubs and larger the fraction, stronger is the overall interaction}, thus, these parameters must be multiplied to represent the inter-layer meta edge weight for the desired interpretation. The domain of this weight will be $(0,1]$ and it will be 1 when every community-wise hub participates in the interaction and all the members from both layers interact with each other. Formally,
\\

\noindent \boldsymbol{$\phi_H$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that,
\begin{enumerate}[label=\roman*.]
\item most of the community-wise hubs participate in the interaction and,
\item larger fraction of member pairs from paired communities are connected, then
\end{enumerate}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight,}

\textit{\centerline{ w(u', v') =  $\frac{|H_{i,j}^{m,n}|}{|H_i^m|}$ * $\frac{|L_{i,j}^{m,n}|}{|V_i^m|*|V_i^n|}$*$\frac{|H_{j,i}^{n,m}|}{|H_j^n|}$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$; $H_i^m$ and $H_j^n$ are set of hubs in $C_i^m$ and $C_j^n$, respectively; $H_{i,j}^{m,n}$ is the set of hubs from $C_i^m$ that participate in the interaction with $C_j^n$; $H_{j,i}^{n,m}$ is the set of hubs from $C_j^n$ that participate in the interaction with $C_i^m$
}
\\

In query 3c. from DBLP, the most active/collaborative authors will be those who are working with most of the other authors in the group, i.e. the degree-based hubs in author communities. Moreover, hubs in conference communities will denote the conferences where large number of research domains are accepted. Thus, hub participation and the requirement for large fraction of publishing authors maps this query to $\phi_H$. Similarly, query 4c from IMDB also gets mapped to $\phi_D$, because most versatile directors and most sought after actors in co-actor groups  correspond to actor community degree hubs and director community degree hubs, respectively and fraction of total number of who-directs-whom interactions needs to be maximized.
\\

In this paper, we have discussed three interpretations of inter-layer interaction. Many more weighting schemes are possible based on the requirements giving rise to different community pairings or 2-communities like hubs based on other centrality metrics, unique fraction of community-wise nodes participating in the interaction and so on. However, the important aspect to be noted here is that the meta-bipartite graph structure need not be recreated while accommodating the new set of weights. These further justifies the advantages of the proposed decoupled approach as the partial layer-wise results can be combined based on \textit{any type} of requirements without having to re-compute any of the layer-wise results. 

\subsection{Discussion on the Community Matches}

Based on the discussed inter-layer interaction interpretations, different community matches will be obtained that will be combined to form the 2-communities. Few characteristics of these resultant 2-communities have been discussed in this section.

\textit{Commutative Property:} The maximal matching algorithm maximizes the flow across the entire network and does not consider the order of the two sets (or layers) in the me. Further, weighing schemes takes into consideration bi-directional nature of interaction. Thus, $C_{i,j}$ = $C_{j,i}$. These results go hand in accordance with the semantics of 2-communities that are also order independent.

\textit{Number of 2-Communities:} For two layers, say $G_i$ and $G_j$ with community sets $C_i$ and $C_j$, respectively the number of community pairings (or 2-communities) will be bounded by min($|C_i|$, $|C_j|$). This is because  

\textit{Ordering the 2-Communities:} Among the 2-communities obtained, higher the weight of the inter-layer meta edges, more is the effect of corresponding interaction interpretation. For example, with respect to $\phi_H$, if a 2-community is obtained such that weight of the inter-layer meta edge is closer to 1, it means that not only \textit{most of the} hubs from both communities are participating in interaction but also the a large fraction of member pairs are also interacting. This means that this community is one of the strongly knit communities, with respect to the interpretation $\phi_H$. Therefore, arranging the 2-communities based on the increasing/decreasing order of inter-layer meta edge weight will give the corresponding community strength/importance order.

\textit{Similarity among the 2-Communities obtained for different choices of $\phi$:}

\begin{comment}



\begin{enumerate}
\item Why is it different in the presence of multiple entities (heterogeneous multilayer networks)?
\item Explain how finding community of the multiplex as a whole will hide a lot of information.
\item Explain through IMDB examples what are the \textit{different} interpretations of a community. Give scenarios.
\item Give the definition with respect to the bipartite based approach, as used in the paper
\end{enumerate}

\subsection{Maximal Matching Approach}
\begin{enumerate}
\item Explain how by using network flow as a subroutine the proposed types of communities be obtained.
\item Explain the modeling of the meta bipartite graph
\item Explain the need for different weighing schemes for finding different types of communities
\item Can we comment on the number of couplings? How to decide the upper bound?
\end{enumerate}

\subsection{Metrics Proposed}
\begin{enumerate}
\item Give reasons of having different weighting schemes are important. Say that these are just few and many more can be defined based on analysis requirement
\item Introduce the 3 classes of metrics that have been used in the paper
\end{enumerate}

\subsubsection{Cumulative Edge Interaction (Metric M(E))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsubsection{Dense Group Interaction (Metric M(D))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsubsection{Hub Interaction (Metric M(H))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsection{Comparison between Metrics}

\begin{enumerate}
\item A given director community may get attached different actor communities based on metrics. 
\item Under what circumstances/conditions do the different metrics give different/same outputs. Can lemmas be stated?
\item From the analytical point of view what does it mean if some couplings comes up as an output using multiple metrics
\item Does ordering the outputs based on metric values give any additional inference? What if the same coupling has different levels of importance in different metrics?
\end{enumerate}
\end{comment}

==> texFiles/Modeling.tex <==
\section{Analysis-Driven Multilayer Network Modeling}
\label{sec:modeling}

%modeling approaches using the data sets to highlight the need for multiplexes as well as the types of multiplexes

%Graphs are the preferred data structure when it comes to modeling datasets where interactions among entities is involved like friendship network among people, collaboration among authors, co-actor relationship and so on. However, most of these interaction networks are defined by multiple types of entities and features, thus giving rise to different possible analysis perspectives. 
For the datasets defined in Section \ref{sec:introduction}, we use a few example analysis queries to identify layers as well as computations needed for the analysis. 

\begin{enumerate}
\item \textbf{UK Accident Data Set}
	\begin{enumerate}[label={\alph*.}]
	\item What are the \textit{accident} prone regions with respect to poor lighting and bad weather conditions? 
    \item How does the \textit{accident} prone regions vary in different parts of the day (6am-9am, 9am-12pm, ...) based on the type of road (roundabout, highway ...) ?
	\end{enumerate}  
\item \textbf{Facebook}
	\begin{enumerate}[label={\alph*.}]
	\item How the \textit{individuals}' age correlate with their comfort level of sharing personal information on social media?
    \item How the \textit{user}-declared political view (e.g., democrat, doesn't care, republican) varies across age groups?
	\end{enumerate}
    \end{enumerate}

%asantra(12/2): Cite Dasfaa-FB? Discuss use of article?
For the required analysis of the above data sets, it can be observed that the relationship among the \textit{same set of entities} is being analyzed, specifically, accident occurrences and FB users, respectively. This indicates that a HoMLN can be used for these two problems. For the accident data set, separation of surrounding conditions into layers makes it easier to analyze these either individually or in arbitrary combinations. Figure~\ref{fig:HoMLN-examples}(a) indicates four such layers on the \textit{same entity set}. Detailed community-based analysis of this data set with respect to the some of the layers shown can be found in~\cite{ICCS/SantraBC17}. Similarly, in the second set of analysis on Facebook, the features are attributed to all people and hence HoMLN is a choice with features separated as layers\footnote{Note that even in this approach, it is possible to have a layer that models combinations of features if that is warranted by the analysis requirements. There is no requirement that each feature is separated into a layer.} Figure~\ref{fig:HoMLN-examples}(b) shows a HoMLN for the Facebook data set with four layers corresponding to different features. More detailed analysis of not only these four layers but additional ones can be found in~\cite{}. Currently, these HoMLNs can be analyzed using either single graph algorithms (by combining all layers into a single layer as a monoplex) or using decoupling-based algorithms for specific compositions as shown in~\cite{ICCS/SantraBC17}.

% make it more crisp - the analysis
\begin{enumerate}[resume]
\label{exa:dblp}
\item \textbf{DBLP (Database Bibliography)}
	\begin{enumerate}[label={\alph*.}]
%sc: i think these two can be slightly modified to correspond to 2 metrics; things like top k pose problems!
%asantra(12/2): can we say that by sorting the output on the metric value we can produce the top-k? Discuss queries
%---------------------
%METRIC 1 (E)
	\item Which are the co-\textit{author} groups who publish in the similar types of \textit{conferences} maximum number of times?
    %\item For the top k research domains, which are the co-\textit{author} groups attending the related \textit{conferences} maximum number of times?
%---------------------
% Metric 2(D) - largest be clear
\item For the largest k research domains, list the tighter co-author groups where most of the authors publish in the related conferences?
%----------------------
%Metric 3(H)
%sc: trying to formulate a hub/participation analysis query
\item Identify the groups of co-authors where the large fraction of authors publishing in the conferences concerned with wide array of research domains include the most active/collaborative ones.
%\item Identify groups of co-authors most of who publish individually in related conferences
%   \item Do the most highly sought after \textit{authors} in each co-author group attend \textit{conferences} belonging to the top research domains? What is the trend across decades?
%----------------------
%HoMLN modeling
\item Compute co-author groups who publish \textit{both} in high ranked conferences \textit{and} journals.
%\item Compute groups of authors who publish as a group \textit{both} in high ranked conferences and similar journals.
	\end{enumerate}
\item \textbf{IMDB (Internet Movie Database)}
	\begin{enumerate}[label={\alph*.}]


%\item Which are the co-actor groups having \textit{maximum interaction} with the directors making movies belonging to top 3 genres? How will actor-director groupings vary if we consider \textit{maximizing the probability of actor-director interaction in group}?
%--------------------------
%METRIC 1(E)
\item Which are the co-actor groups having \textit{maximum interaction} with similar directors?

%----------------------
% METRIC 2(D)
    \item List the tight co-actor groups most of whom who have worked with directors making movies in the most popular genres
%----------------------
% METRIC 3(H)
\item Which are the most versatile directors who work the most sought after actors apart from other actors in co-actor groups ?
%\item Which are the movie genres being opted for by the directors with whom the most sought after actor from co-actor groups are working?
%\item What is the average rating of the movies in which the most sought after actors from the co-actor groups work in?
%Do the actors and directors who are \textit{most sought after} in their respective groups interact with each other?    
%----------------------
% HoMLN Modeling
\item What are the co-actor groups working in \textit{both} Comedy \textit{and} Drama genres?
	\end{enumerate}
\end{enumerate}

In contrast to the earlier two data sets, in case of the IMDB data set, in addition to features, \textit{multiple entity types (e.g., person as a director/actor/writer, movies)  are being analyzed}. Similarly, in case of the DBLP data set, multiple entity types are present (e.g., authors, conferences, cities). Note that each of these entity types have their own features (e.g., movies having a rating) as well as entity types may also have relationships (director directing an actor). The same is true for the DBLP data set.

To illustrate, analysis a), b) and c) of the DBLP data set, co-authors can be represented as a layer and conferences in related research domains as another layer. Authors publishing in specific conferences form inter-layer edges. Similarly, for the IMDB dataset, the analysis a), b) and c) can be taken care of by modeling the co-actors as one layer and the directors linked to each on the basis of the similarity of movie genres they are involved with as another layer. Actors being directed by specific directors make the inter-layer edges. These analysis translate to finding communities in each layer and finding matches across layers among communities based on inter-layer edges. However, the semantics of the analysis is slightly different in that a) considers the maximum interaction, b) considers the largest groups and c) considers the most sought after participants.  

%The semantics of analysis c) of the DBLP data set is slightly different in that it is asking for combined communities who not only publish as a group, but also individually.

On the other hand, analysis of d) for the DBLP data set and IMDB data set can be modeled as Homogeneous MLN, as they deal with analyzing different interactions among the same set of entities, i.e. authors and actors, respectively. For DBLP, the authors form a single entity set and each layer corresponds to co-authors who publish in different conferences (ICDM, ICDE, KDD, ...) and journals (VLDB Journal, TKDE, ...), respectively. On the other hand, for IMDB, the actors become the entity set and any two actors are connected in each layer if they have co-acted in movie that belonged to a specific genre (Comedy, Action, Drama, Thriller, ...). These analysis can be performed using the approaches proposed in~\cite{ICCS/SantraBC17}.

To summarize, multiplex (all three kinds) characteristics and their relationship to modeling can be understood clearly and appreciated if we view a multiplex as a meta graph. Treating each layer as a node and the presence of inter-layer edges as an edge, HoMLN is a clique and HeMLN is a forest of connected graphs. Any analysis uses (or corresponds to) a connected subgraph in this meta graph. 

%Similar modeling can be done for the IMDb data set. We illustrate it as part of the experimental analysis section (Section~\ref{sec:experiments}).

\begin{comment}
Moreover, the highlighted example queries also show that different combinations of features will be required to obtain the desired inferences about the same or different sets of entities. Such complex multi-feature datasets that need to be flexibly analyzed are modeled using a \textit{network of networks} known as multilayer networks or multiplexes, broadly categorized as homogeneous or heterogeneous \cite{BDA/SantraB17}.

\begin{wrapfigure}{l}{0.6\textwidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/HoMLN-example}
\caption{Homogeneous Multiplex Examples}
	\label{fig:HoMLN-examples}
\end{wrapfigure}

Homogeneous multiplexes are the ones where the set of nodes (denoting entities) is same in each network (or layer), but are connected by edges if they are related/interact/are similar based on a particular feature. That is, the set of intra-layer edges varies. Due to the presence of same set of nodes in each layer, there is no explicit need of inter-layer edges. For example, Figure \ref{fig:HoMLN-examples} (a) shows an example accident multiplex for 5 accident occurrences that are connected if they are similar with respect to light conditions ($G_1^1$), weather conditions ($G_1^2$), road type ($G_1^3$) or time of the day ($G_1^4$). Similarly, Figure \ref{fig:HoMLN-examples} (b) illustrates a Facebook multiplex that connects FB users based on age ($G_2^1$), privacy concern ($G_2^2$), political view ($G_2^3$) and friends ($G_2^4$).

\begin{wrapfigure}{r}{0.6\textwidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/HeMLN-example}
\caption{Heterogeneous Multiplex Examples}
	\label{fig:HeMLN-examples}
\end{wrapfigure}

On the other hand, in case of heterogeneous multiplexes the set of nodes (or entities) in each network (or layer) is different. Thus, apart from intra-layer edges, such a multiplex also has inter-layer edges connecting nodes from different sets. For example, for the DBLP multiplex shown in Figure \ref{fig:HeMLN-examples} (a), the authors are connected if they co-authored at least one paper ($G_3^1$) and the conferences are connected if they belong to similar research domain ($G_3^2$). Moreover, authors are connected to the conferences they have published in. Similarly, in the IMDB multiplex (Figure \ref{fig:HeMLN-examples} (b)), actors who have co-acted in atleast one movie ($G_4^1$) and directors directing similar movie genres are connected to each other ($G_4^2$). The inter-layer edge in this case represent the who-directs-whom relationship.

Some interesting insights can be obtained in such datasets by detecting the most tightly connected group of entities, most influential entity, hidden motifs with respect to different combinations of features. Considerable amount of work has been done in analyzing homogeneous multiplexes. In our earlier work, we have proposed the combination of layers (or networks) using Boolean compositions like AND (intersection of layer-wise edges), OR (union of layer-wise edges) and NOT (complement of the edge set of a layer). Moreover, a principled approach  has been proposed for finding communities (\cite{ICCS/SantraBC17}) or hubs (\cite{ICDMW/SantraBC17}) for a combined network by just using the communities or hubs from the individual layers using Boolean operations. This approach is computationally efficient as it saves space and time needed to separately generate and analyze different possible combined networks. For example, to answer query 1a one will need find communities of the combined AND network, $G_{1}^{1AND2}$, which will translate to the accident prone regions with respect to similar light and weather conditions. Using the proposed approach, we will just have to use the communities from Light ($G_1^1$) and Weather ($G_1^2$) layer. Similarly, answering of the query 2b will need just the communities from Age ($G_2^1$) and Political View ($G_2^2$) layer.

On the other hand, the work in the area of heterogeneous multiplexes is minimal. Even the definition of community in such a multiplex is not well defined. In this paper, we explore the community-based analysis of a complex dataset modeled as a heterogeneous multiplex. In the next section, we provide the different interpretations of a heterogeneous community and propose metrics that can quantify the interpretations. We will take cue from our work for homogeneous multiplexes, by using the re-using the communities from the individual layers and combining them as per analysis requirement. Even though the work provided is generalized, we will use the IMDB dataset for motivating the modeling and community-based analysis schemes.
\end{comment}

==> texFiles/allcites-RelatedWork_2.tex <==
\section{Related Work}
\label{sec:related-work}

As the focus of this paper is community definition and its efficient detection in HeMLNs, we present relevant work on simple graphs and MLNs. The advantages of modeling using MLNs are discussed in~\cite{Boccaletti20141,CommSurveyKimL15, MultiLayerSurveyKivelaABGMP13}.
%% BDA/SantraB17,

\textit{Community detection} on a simple graph involves identifying groups of vertices that are more connected to each other than to other vertices in the network. Most of the  work in the literature considers \textbf{single networks or simple graphs} where this objective is translated to optimizing network parameters such as modularity ~\cite{clauset2004} or conductance ~\cite{Leskovec08}. As the combinatorial optimization of community detection is NP-complete ~\cite{Brandes03}, a large number of competitive approximation algorithms have been developed (see reviews in ~\cite{ Xie2013}.) %%Fortunato2009,
Algorithms for community detection have been developed for different types of input graphs including directed ~\cite{Yang10}, %%, Leicht08
edge-weighted ~\cite{Berry2011}, and dynamic networks~\cite{porterchaos13}. %%,Bansal201
%Recently there have also been algorithms for identifying overlapping communities~\cite{Yang2013acm,Chakraborty2015a}.
However, to the best of our knowledge, there is no  community definition and detection that include node and edge labels, node weights as well as graphs with self-loops and multiple edges between nodes\footnote{This is in contrast to subgraph mining, search, and querying of graphs where non-simple graphs are widely used.}.
%%In contrast, subgraph mining~\cite{datamine/KuramochiK05,KDD/HolderCD1994, tkde/DasC18}, querying~\cite{tkde/JayaramKLYE15,dawak/DasGC16}, and search~\cite{bigdataconf/HaoC0HBH15,pods/ShashaWG02} have used graphs with node and/or edge labels including multiple edges between nodes, cycles, and self-loops.}. 
Even the most popular community detection packages such as Infomap \cite{InfoMap2014} or Louvain~\cite{DBLP:Louvain}, do not accept non-simple graphs. 

Recently, community detection algorithms have been extended to \textbf{HoMLNs}. Algorithms based on matrix factorization \cite{dong2012clustering}, %%,qi2012community
pattern mining \cite{silva2012mining}, %%,zeng2006coherent
cluster expansion philosophy \cite{li2008scalable}, Bayesian probabilistic models \cite{xu2012model}, regression \cite{cai2005mining}, spectral optimization of the modularity function based on the supra-adjacency representation \cite{zhang2017modularity} and a significance based score that quantifies the connectivity of an observed vertex-layer set
through comparison with a fixed degree random graph model \cite{wilson2017community} have been developed. However, all these approaches \textit{analyze a MLN either by aggregating all (or a subset of) layers (straightforward for a HoMLN using Boolean and other operators) or by considering the entire multiplex as a whole}. 
%%Recently a decoupling-based approaches for detecting communities~\cite{ICCS/SantraBC17} and centrality~\cite{ICDMW/SantraBC17} in HoMLN have been proposed. 
%The decoupling approach uses partial results from individual layers and  composes them for Boolean operators to compute communities for combinations of layers. This approach is more efficient as it avoids re-computation of layer communities and provides  flexibility for analysis. This approach nicely leverages the algorithms developed for a single network. 
%%They reduce the exhaustive analysis complexity from O($2^N$) (for all possible subsets of layers) to linear complexity for \textit{N} layers by composing combinations of them. The goal of this paper is to do the same for HeMLNs.

%allows the flexible analysis of any complex dataset modeled as a homogeneous multilayer network in a cost-effective manner as one does need to to generate and separately analyze the combined networks (close to O($2^N$) in an exhaustive analysis, if the multiplex has N layers).

Majority of the work on analyzing HeMLN (reviewed in \cite{shi2017survey,sun2013mining}) focuses on developing meta-path based techniques for determining the similarity of objects~\cite{wang2016relsim}, classification of objects~\cite{wang2016text}, predicting the missing links~\cite{zhang2015organizational}, ranking/co-ranking~\cite{shi2016constrained} and recommendations~\cite{shi2015semantic}. An important aspect to be noted here is that most of them do not consider the intra-layer relationships and concentrate mainly on the bipartite graph formed by the inter-layer edges. %Further, they either consider the multilayer network as a whole or remove the type information of nodes or project one layer onto another while proposing the approaches, thus neglecting the effect of different combinations

%%In contrast to the homogeneous case, there \textbf{is no consensus on the definition of a community, let alone structure-preserving} for \textbf{HeMLNs}. 
The type-independent~\cite{LayerAggDomenicoNAL14} and projection-based~\cite{Berenstein2016} approaches used for HeMLNs do not preserve the structure or semantics of the community. The type independent approach collapses  all layers into a simple graph keeping \textit{all} nodes and edges (including inter-layer edges) sans their types and labels. Similarly, the projection-based approach projects the nodes of one layer onto another layer and uses the layer neighbor and inter-layer edges to collapse the two layers into a single graph with a single entity type instead of two. The presence of different sets of entities in each layer and the presence of intra-layer edges makes structure-preserving definition more challenging for HeMLNs and also warrants a composition technique (as proposed in this ppaer.) A few existing works have proposed techniques for generating clusters of entities \cite{melamed2014community}, but they have only considered the inter-layer links and not the networks themselves. Thus, the \textit{combined effect of layer communities, entity types, intra- and inter-layer relationships (types) have not been included in defining a community in a HeMLN}.  This paper hopes to fill that gap.

%%This is very much needed for mapping analysis requirements that require community-based computations when a data set is modeled as a heterogeneous MLN.

%This paper proposes a decoupling approach to community detection in HeMLNs. As in~\cite{ICCS/SantraBC17}, the goal is to use partial results from each layer and compose them to detect communities for a given set of layers. As we demonstrate, unlike the homogeneous MLNs, the analysis semantics plays a role in the composition of layers in terms of the choice of metrics used for composition. 
%In this paper, we will \textit{focus on proposing decoupling-based approaches for determining heterogeneous communities}.

==> texFiles/m-and-c-alternatives.tex <==
\section{Modeling and Analysis Alternatives}
\label{sec:alternatives}

Research on graph-based modeling and analysis have been around for a long time. In addition to analysis~\cite{}, search and querying of graphs are also becoming mainstream~\cite{DBLP:conf/cikm/MassS14,bu2014integrating}. As the size of the data sets increases and their characteristics become more complex, scalable approaches are being developed to cope with the increase in data size and complexity using partitioning and parallel processing techniques. Partitioned approaches with loss-less computation as well as fast approximate algorithms are being investigated~\cite{}.

In the above backdrop, this paper briefly addresses modeling alternatives for data sets that can be characterized as multiple entity and feature types as well as approaches for analyzing these models.

\subsection{Modeling Alternatives}

%asantra(2/11): discuss 3
In this paper, we consider \textit{three alternatives to model a complex data set using graphs}. We introduce them informally here and then define them formally in Section~\ref{sec:problem-statement}. The \textit{traditional approach (termed single graph or simple graph or ordinary graph or a monoplex)} models entities as nodes (including labels) and relationship based on features as edges (including labels and/or weights, if present) of the graph. This model gives rise to graphs with single node types (if entity types are not distinguished even when multiple node types are modeled using this approach) and single edges between nodes (either for a single feature or for a combination of features) with or without edge weights. More details of the data set can be captured using this model by including node types in terms of labels (and even multiple labels) and multiple edges corresponding to relationships corresponding to different features again with or without labels and/or weights (termed attribute graphs in the literature.) There are several algorithms for analyzing graphs, such as detecting cliques, communities, hubs, mining subgraphs, triangles etc. Most of these are applied on the entire graph and typically ignore labels in the graph (except in subgraph mining); also most of the algorithms do not handle multiple edges between nodes and their weights as well as labels while doing the analysis. In order to use these algorithms, one may have to separate graphs if analysis need to be performed on a subgraph with specific node and edge characteristics (e.g., specific labels.) 

In order to use extant monoplex algorithms, a single graph (i.e., single edges between nodes, and only one type of nodes) may have to be created even for data sets with multiple entity and features types. Although combining features is possible, it is not straightforward. If features are of different types (e.g., numerical and categorical),  combining them in a meaningful way may not be that easy. In addition, assigning importance to different features could be daunting as well. Finally, if one wants to analyze a subset of entities and associated feature types, separate simple graphs have to be created (or separated) for each such combination or analysis. Based on the above, in this paper, we argue for the appropriateness of a \textit{\textbf{M}ulti\textbf{L}ayer \textbf{N}etwork (or \textbf{MLN}) for both modeling and analyzing multi entity and feature data sets}. 
%Further, we use three types of multiplexes -- homogeneous, heterogeneous, and hybrid -- that are useful for modeling data sets based on analysis needs \cite{BDA/SantraB17}. 

\sharma{2/8/2019}{need to confirm these term usages are consistent with the literature!}
%asantra(12/2): discuss multiplex/MLN?

A MLN (used interchangeably with a multiplex\footnote{We use the term multiplex when we do not differentiate between the entity types in the layers of multiplexes and use abbreviated names -- HoMLN for homogeneous, HeMLN for heterogeneous, and HyMLN for hybrid MLNs when types are relevant.}) is a collection of layers whose nodes are connected within each layer and in addition, nodes from different layers can also be connected. The choice and semantics of nodes for modeling layers and intra-layer edges as well as inter-layer edges are analysis-driven. Layers are formed based on the analysis requirements with respect to the number of features used/needed. Once the layers are formed, they can be analyzed for feature-wise and aggregate (combinations of feature and/or entity types) analysis. It is easy to visualize that in some multiplexes, the node sets are the \textit{same in all layers.} Accident data set is an example of a data set where nodes in each layer are the same (accident as individual occurrence or geographical close to each other grouped as one)% -- within a specified radius)
and each layer represents a relevant feature (light, weather, road,...) with respect to an accident. In each layer, two accidents whose corresponding features are similar are connected with an edge. This type of multiplex where each layer has the same set and type of nodes is termed a \textbf{Ho}mogeneous \textbf{M}ulti\textbf{L}ayer \textbf{N}etwork or \textbf{HoMLN}. The inter-layer edges are implicit as the node sets of all layers are identical and are not drawn. Figure~\ref{fig:HoMLN-examples} shows examples from the accident and Facebook data sets.

%sc; was .6 earlier; changed to 0.5
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/HoMLN-example-1}
\caption{Homogeneous MLN Examples of Accident and Facebook Data Sets}
\label{fig:HoMLN-examples}
\end{figure}

Another alternative is to model a data set, again, using layers except that each layer has a different entity type as its nodes. The graph of a layer is defined with respect to chosen features and entity types. In this case, the inter-layer links are not implicit, but are defined explicitly based on a relevant feature that corresponds to an edge. This type of multiplex where each layer has a different set and type of nodes is termed a \textbf{He}terogeneous \textbf{M}ulti\textbf{L}ayer \textbf{N}etwork or \textbf{HeMLN}. Figure~\ref{fig:HeMLN-examples} shows examples from the DBLP and IMDB data sets. Again the choice of HoMLN or HeMLN is driven by the data set and analysis needs. It is possible to model the \textit{same data set} using both of the above alternatives depending on the analysis needs.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/HeMLN-example-1}
\caption{Heterogeneous MLN Examples of DBLP and IMDb Data Sets}
	\label{fig:HeMLN-examples}
\end{figure}

%The inter-layer edges and the entity types add complexity to the aggregate analysis. 
It is also possible to have a combination of these two types of multiplexes for a given data set and is termed a \textbf{Hy}brid \textbf{M}ulti\textbf{L}ayer \textbf{N}etwork or \textbf{HyMLN}. For example, combining Facebook information with actor and director information results in a hybrid MLN.

\subsubsection{Observations}

From a modeling perspective, especially for a data set with multiple entity and features types, we argue that a MLN is a better choice in many ways. First, modeling using a single attribute graph (traditional approach) is possible, clarity is lost. Separation of features and node types are not possible. Furthermore, as we indicate below in the analysis alternatives, individual or aggregate analysis and their computation is difficult as most of the extant algorithms deal only with simple graphs. On the other hand, MLNs allow features to be separately modeled as a layer for understanding and more importantly each layer can be analyzed using extant algorithms. As we shall see later, MLN modeling is also amenable to parallel processing. There are other advantages as well for this modeling. It affords flexibility for combining of features for aggregate analysis as discussed below.

\subsection{Analysis alternatives}
Once the data set is modeled using any of the MLN alternatives, the goal is to develop efficient algorithms for computing communities\footnote{In this paper, we delimit ourselves to \textit{communities} in HeMLNs. Other types of analysis, such as centrality, subgraph mining, even querying and search are applicable.}.

%asantra(12/2): discuss? rephrase
If the model is a simple graph, a large number of algorithms for community detection are available (e.g., Infomap~\cite{{InfoMap2014}}, Louvain~\cite{DBLP:Louvain} being prominent ones) which can be directly used. If the model is an attributed graph, the choice of computations is limited (or even not available) depending upon the analysis to be performed. Computationally, the alternatives for a single graph approach are: i) combine features in some way and use extant single graph approaches, ii) separate entities and features as desired, ignore their types and apply single graph algorithms. The main advantage of this choice for modeling is that we can leverage a variety of algorithms and packages currently available for detecting communities. However, ignoring types in aggregate analysis may result in loss of information or precision of analysis (as will be discussed later in the paper.) 

On the other hand, modeling using a MLN can still leverage single graph algorithms on each layer independently. This is a huge advantage of the proposed approach. If this is to be leveraged for aggregate analysis, techniques need to be developed to combine partial results from each layer. This has to be done either in a loss-less manner or with high or bounded accuracy. This is the primary challenge for using this modeling alternative. Modeling in terms of layers provides a natural "divide and conquer" capability which is amenable to parallel processing as well. With the availability of layers, combinations of features can be analyzed without having to re-create a new graph for each such analysis which is exponential in the number of features to be handled. Also, combining partial results is likely to be computationally small as compared to layer analysis. Hence, efficiency can also be significantly improved using this modeling if efficient concomitant composing functions are developed.

Due to its modeling advantages, currently approaches are being developed for the analysis of MLNs as it provides flexibility for selecting combinations of layers and efficiency. When data sets are modeled using MLNs, there are several alternatives for analysis: i) aggregate or combine desired number of layers of a MLN as a single graph and process using existing algorithms,  ii) process the entire multiplex as a whole (without reducing it to a single graph), and iii) keep them as layers and process desired number of layers using partial results and a composition function. Approach i)  is not desirable as it negates the advantages of the MLN model and approach ii) requires development of new algorithms~\cite{yao2014pathsimext,wang2016relsim} that have to traverse back and forth across layers making them difficult to parallelize and scale. In our view, approach iii) discussed in the rest of the paper is likely to be flexible, efficient, and scalable as discussed in the rest of the paper for HeMLNs. The computation complexity to the first alternative.

\subsubsection{Observations}

Modeling alternatives give rise to new computational challenges as discussed above. In spite of that, we argue that overcoming these challenges will result in solutions to big data analysis that are flexible, efficient, and scalable. Once the layers have been identified and their analysis is available, computing "what-if" analysis is quite straightforward. Even if modeling results in multiple sets of MLNs, analysis can be performed across layers from different MLNs equally easily. Furthermore, updating the data set results in updating corresponding layers and recomputing only updated layers. Even here incremental techniques (existing and new ones) can be applied.  Temporal analysis is possible by creating MLNs for desired periods and they can be cross analyzed without incurring expensive computations again. In summary, the proposed approach has significant benefits as compared to the alternatives.



==> texFiles/old-Detection.tex <==
\begin{comment}
\section{Extending Heterogeneous Community Detection to k layers}
\label{sec:extensions}

In Section \ref{sec:hemln-community}, we discussed about how to generate a community involving two types of entities based on the inter-layer interaction interpretation. Here we will extend the proposed decoupling based approach to k layers by explaining the details of join-based step that combines the pair-wise community matches, i.e. 2-communities to produce the k-community in Section \ref{sec:join}, followed by a discussion on the characteristics of a k-community in Section \ref{sec:k-comm-char}.

\subsection{Detecting k-communities using Pair-wise Join based Approach}
\label{sec:join}

\subsection{Discussion on k-communities}
\label{sec:k-comm-char}

\begin{enumerate}
\item Different ways of composing the pair-wise community results
\item Provide intuition behind our approach. State different analysis examples that use 3 layers from IMDB
\item Give the join and decoupling based algorithm to extend the community detection to k layers.
\item Is it commutative and associative? Depends on the analysis question.
\item Comment about mix and match of different metrics as well. However that has not been explored in this paper. State assumptions clearly
\end{enumerate}

\end{comment}


\section{Community Detection in HeMLNs}

In this section, we dwell into the problem of detecting communities for two layers, say $G_i$ and $G_j$ that are connected based on the bipartite graph, $X_{i,j}$. With respect to the entities from these two layers, there are three types of interactions a) interaction among the entities in layer $G_i$, b) interaction among the entities in layer $G_j$ and c). interaction between the entity sets from $G_i$ and $G_j$. %In order to obtain strongly knit groups of 2 different entities, i.e. 2-communities these three interactions need to be maximized among the group members. Applying the existing community detection techniques by removing the node and edge type information and considering the multiplex as a whole will
Informally, a strongly knit group of 2 different entities, i.e. 2-community, that \textit{preserves the entity types and relationships among them}, must be such that all \textit{these three interactions are maximized among its members, separately}. Maximizing the interactions among entities of same type (as in a) and c)) translates to the layer-wise communities (in layers $G_i$ and $G_j$). Further, maximizing the interactions between entities from two different sets translates to an optimal pairing of communities from two layers. However, this pairing of communities depends on the analysis requirements that lead to \textit{inter-layer interpretations} like maximizing a specific \textit{proportion} of interaction, maximizing interaction among community members \textit{satisfying a graph property} and so on. Based on this discussion, the formal definition for a 2-community has been given below,

\noindent\textbf{2-Community:} \textit{For a chosen inter-layer interpretation, $\phi$, $C_{i,j}^r(V_i^r, E_i^r, V_j^r, E_j^r, E_{i,j})$ is a 2-community with respect to $G_i$ and $G_j$, if a). $C_i^r(V_i^r, E_i^r)$ is a community in $G_i$, b). $C_j^r(V_j^r, E_j^r)$ is a community in $G_j$ and c). maximizing $\phi$ leads to the pairing of $C_i^r$ and $C_j^r$}.

\begin{algorithm}
\caption{Algorithm for 2-Community Detection}
\label{algo:2-community}
\begin{algorithmic}[1]
   \REQUIRE $C_i$: Set of Communities from $G_i$, $C_j$: Set of Communities from $G_j$ , $X_{i,j}$, $\phi$, $C_{i,j}$ = $\emptyset$

Generate the Meta-bipartite graph, $X'_{i,j}(V'_i, V'_j, L'_{i,j})$
   \STATE $V'_i$ = $\emptyset$, $V'_j$ = $\emptyset$, $L'_{i,j}$ = $\emptyset$
   \FORALL {$C_i^m \in C_i$}
       \STATE $V'_{i} \gets V'_{i} \cup u'_m$
   \ENDFOR
   
    \FORALL {$C_j^m \in C_j$}
       \STATE $V'_{j} \gets V'_{j} \cup v'_m$
   \ENDFOR

    \FORALL {$u'_m \in V'_i$}
    	    \FORALL {$v'_n \in V'_j$}
            \IF {$\exists$a,b: ($u_a$, $v_b$) $\in$ $X_{i,j}$, where, $u_a$ $\in$ $C_i^m$ and $v_b$ $\in$ $C_j^n$}
       \STATE $X'_{i,j} \gets X'_{i,j} \cup (u'_m, v'_n)$            \ENDIF
            \ENDFOR

   \ENDFOR
    \FORALL {$(u'_m, v'_n) \in X'_{i,j}$}
       \STATE Assign weight, $w(u'_m, v'_n)$, based on $\phi$
   \ENDFOR
   
   \STATE Apply Maximal Matching Algorithm to get 2-community set, $C_{i,j}$
\begin{comment}


   \FORALL {$u_m^{k} \in V_{k}$}
       \STATE $V_{k'} \gets V_{k'} \cup u_m^{k'}$
   \ENDFOR

   \FORALL {$ u_m^{k'}, u_n^{k'} \in V_{k'}, m > n$}
       \IF {$(u_m^{k}, u_n^{k}) \notin E_{k}$}
           \STATE $E_{k'} \gets E_{k'} \cup (u_m^{k'}, u_n^{k'})$
       \ENDIF
   \ENDFOR
\end{comment}
\end{algorithmic}
\end{algorithm}


% meta node has its own characteristics and that will effect the weight of the edge. draw relations from couple matching. intuition behind giving weights. different from traditional max flow. node semantics into the flow

% HemLN is a forest. each analysis requires a connected subgraph. and then detect communities

\subsection{Detecting 2-communities using Maximal Flow based Matching Approach}
\label{sec:flow}

An optimal matching of the layer-wise communities is required such that the chosen interpretation of the inter-layer interaction is maximized. In bipartite graphs, maximum flow-based matching algorithms like Ford-Fulkerson give a set of pairings such that the overall flow across the network is maximized \cite{}. Thus, by generating a \textit{meta-bipartite graph} where the layer-wise communities become two sets of meta nodes which are connected by a meta edge if any of the members of meta nodes from different sets are connected in the actual multiplex, this problem can be mapped to a network flow problem. Therefore, based on the inter-layer interpretation, $\phi$, derived from the analysis requirements, if appropriate weights are specified on the inter-layer meta edges such that the \textit{optimal matching of communities is obtained that will be combined to form the 2-communities}. 


Algorithm \ref{algo:2-community} gives the process to detect 2-communities for layers, $G_i$ and $G_j$ for the chosen inter-layer interpretation, $\phi$.
A decoupling-based approach is followed for detecting communities for 2 layers, where the layer-wise communities are generated only once and combined as required. Based on the analysis requirements, a meta-bipartite graph, $X'_{i,j}(V'_i, V'_j, L'_{i,j})$, is formed using the communities from $G_i$ and $G_j$ that are treated as meta nodes for the two sets ($V'_i, V'_j$) who are connected by inter-layer meta edges ($L'_{i,j}$) such that any of the member pairs from the communities is connected. Weights are specified on the inter-layer meta edges based on the inter-layer interpretation, $\phi$. Network flow algorithm is applied on this graph to obtain the community pairings that are combined to form the 2-community. Next we will discuss the various interpretations of inter-layer interaction maximization.

\subsection{Inter-layer Interaction Interpretation ($\phi$) Classes}
Based on the requirements of the analysis, the interaction between the entities of different types can have multiple interpretations. In this paper, broadly we have discussed three classes of interpretations based on aggregation of interaction (Sec \ref{sec:m1}), density of interacting communities (Sec \ref{sec:m2}) and participating hubs in the interaction (Sec \ref{sec:m3}). In this section, we discuss how these different interpretations will effect the weights of the inter-layer meta edges in the meta-bipartite graph such that the maximal flow based matching algorithms give the community pairings with desired characteristics. Moreover, we will show how the requirements of the queries listed in Section \ref{sec:modeling} can be mapped on one of these. 

\subsubsection{Aggregate Interaction ($\phi_A$)}
\label{sec:m1}
Certain queries will need the detection of groups where apart from strong interaction among the same type of entities, \textit{maximum interaction exists among entities from different sets}. Therefore, in this case, weight of the inter-layer meta edges should reflect number of interactions that exist between the members of every community pair from two layers.  Formally,
\\

\noindent \boldsymbol{$\phi_A$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that
\begin{itemize}
\item maximum number of member pairs from paired communities are connected, then
\end{itemize}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight, }

\textit{\centerline{w(u', v') =  $|L_{i,j}^{m,n}|$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$
}
\\

Query 3a. from DBLP and query 4a. from IMDB fall under this class where maximum number of author-conference connections and actor-director connections need to be considered for answering the query.

\subsubsection{Dense Community Interaction ($\phi_D$)}
\label{sec:m2}
Another class of queries will require the larger fraction of the members belonging to the \textit{dense entity groups} from both the layers to interact. In contrast to $\phi_A$, here the layer-wise community characteristics will play a role in the matching. Apart from that, instead of \textit{number} of interactions, this interpretation takes into account the \textit{fraction} of total member pairs from communities that are interacting. Clearly, \textit{higher the densities and larger the fraction, stronger is the interaction among same and different types of entities, respectively}. Thus, the directly proportional behavior of these parameter shows that they must be multiplied to represent the inter-layer meta edge weight for this interpretation. The domain of this weight will be $(0,1]$ and it will be 1 when both the communities are cliques and all the members from both layers interact with each other. Formally,
\\

\noindent \boldsymbol{$\phi_D$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that,
\begin{enumerate}[label=\roman*.]
\item dense communities are paired and,
\item larger fraction of member pairs from paired communities are connected, then
\end{enumerate}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight,}

\textit{\centerline{ w(u', v') =  $\frac{2*|E_i^m|}{|V_i^m|*(|V_i^m|-1)}$ * $\frac{|L_{i,j}^{m,n}|}{|V_i^m|*|V_i^n|}$*$\frac{2*|E_j^n|}{|V_j^n|*(|V_j^n|-1)}$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$.
}
\\

In query 3b. from DBLP, the largest research domains will correspond to the densest communities from conference layer and tight co-author groups will be the dense communities from author layer. Thus, along with the requirement to check whether \textit{most of the members} of co-author publish in similar conferences, this query complies with the specifications of $\phi_D$. Similarly,  query 4b from IMDB also gets mapped to $\phi_D$, as tight co-actor groups and most popular genres correspond to communities in actor and director, respectively and fraction of total number of who-directs-whom interactions needs to be maximized.



\subsubsection{Hub Interaction ($\phi_H$)}
\label{sec:m3}
The third class of queries that we have considered will require that apart from a \textit{large fraction of the interacting member pairs}, the \textit{most central entities} from each group also interact across layers. Thus, here the inter-layer interaction takes into consideration the number of community-wise hubs that participate in the interaction. High centrality nodes (or hubs) can be defined based on metrics like degree centrality (vertex degree), closeness centrality (mean distance of the vertex from other vertices), betweenness centrality (fraction of shortest paths passing through the vertex), and eigenvector centrality. In this paper, we have used degree centrality as the metric. Similar to $\phi_D$, as \textit{higher the ratio of participating hubs and larger the fraction, stronger is the overall interaction}, thus, these parameters must be multiplied to represent the inter-layer meta edge weight for the desired interpretation. The domain of this weight will be $(0,1]$ and it will be 1 when every community-wise hub participates in the interaction and all the members from both layers interact with each other. Formally,
\\

\noindent \boldsymbol{$\phi_H$}: \textit{If communities from layer $G_i$ and $G_j$ need to be matched such that,
\begin{enumerate}[label=\roman*.]
\item most of the community-wise hubs participate in the interaction and,
\item larger fraction of member pairs from paired communities are connected, then
\end{enumerate}
for every $(u', v')$ $\in$ $L'_{i,j}$, where u' and v' denote the communities, $C_i^m$ and $C_j^n$ in the meta-bipartite graph, respectively, the weight,}

\textit{\centerline{ w(u', v') =  $\frac{|H_{i,j}^{m,n}|}{|H_i^m|}$ * $\frac{|L_{i,j}^{m,n}|}{|V_i^m|*|V_i^n|}$*$\frac{|H_{j,i}^{n,m}|}{|H_j^n|}$,}
}
\textit{\noindent where $L_{i,j}^{m,n}$ = $\bigcup_{u \in C_i^m, v \in C_j^n}\{(u, v): (u, v) \in L_{i,j}\}$; $H_i^m$ and $H_j^n$ are set of hubs in $C_i^m$ and $C_j^n$, respectively; $H_{i,j}^{m,n}$ is the set of hubs from $C_i^m$ that participate in the interaction with $C_j^n$; $H_{j,i}^{n,m}$ is the set of hubs from $C_j^n$ that participate in the interaction with $C_i^m$
}
\\

In query 3c. from DBLP, the most active/collaborative authors will be those who are working with most of the other authors in the group, i.e. the degree-based hubs in author communities. Moreover, hubs in conference communities will denote the conferences where large number of research domains are accepted. Thus, hub participation and the requirement for large fraction of publishing authors maps this query to $\phi_H$. Similarly, query 4c from IMDB also gets mapped to $\phi_D$, because most versatile directors and most sought after actors in co-actor groups  correspond to actor community degree hubs and director community degree hubs, respectively and fraction of total number of who-directs-whom interactions needs to be maximized.
\\

In this paper, we have discussed three interpretations of inter-layer interaction. Many more weighting schemes are possible based on the requirements giving rise to different community pairings or 2-communities like hubs based on other centrality metrics, unique fraction of community-wise nodes participating in the interaction and so on. However, the important aspect to be noted here is that the meta-bipartite graph structure need not be recreated while accommodating the new set of weights. These further justifies the advantages of the proposed decoupled approach as the partial layer-wise results can be combined based on \textit{any type} of requirements without having to re-compute any of the layer-wise results. 

\subsection{Discussion on the Community Matches}

Based on the discussed inter-layer interaction interpretations, different community matches will be obtained that will be combined to form the 2-communities. Few characteristics of these resultant 2-communities have been discussed in this section.

\noindent\textbf{Commutative Property:} The maximal matching algorithm maximizes the flow across the entire network and does not consider the order of the two sets (or layers) in the computation. Further, weighing schemes take into consideration the bi-directional nature of interaction. Thus, $C_{i,j}$ = $C_{j,i}$. These results are in accordance with the semantics of 2-communities that are also order independent.

\noindent\textbf{Number of 2-Communities:} For two layers, say $G_i$ and $G_j$ with community sets $C_i$ and $C_j$, respectively the number of community pairings (or 2-communities) will be bounded by min($|C_i|$, $|C_j|$). This is because  

\noindent\textbf{Ranking the 2-Communities:} Among the 2-communities obtained, higher the weight of the inter-layer meta edges, more is the effect of corresponding interaction interpretation. For example, %with respect to $\phi_H$, if a 2-community is obtained such that weight of the inter-layer meta edge is closer to 1, it means that not only \textit{most of the} hubs from both communities are participating in interaction but also the a large fraction of member pairs are also interacting. This means that this community is one of the strongly knit communities, with respect to the interpretation $\phi_H$.
with respect to $\phi_A$, if a 2-community is obtained such that weight of the inter-layer meta edge is \textit{highest among all the matchings}, then it implies that these two communities have the maximum interaction as compared to any other community pair. Thus, this community will be the most strongly knit community, with respect to the interpretation $\phi_A$.
Therefore, arranging the 2-communities based on the increasing/decreasing order of inter-layer meta edge weight will give the corresponding community strength/importance order.

\noindent\textbf{Comparing 2-Communities obtained from different choices of $\phi$:} Under certain circumstances, depending on the graph characteristics of the HeMLN, it might be possible that a 2-community is obtained for multiple interpretations of the inter-layer interaction.

\textbf{\textit{Lemma 1.1}}
\textit{If the inter-layer meta edge weights are in the same proportion for different choices of $\phi$, then the same set of 2-communities will be obtained.}
%\vspace{-10pt}
\begin{proof}
The structure for meta-bipartite graph is fixed for any $\phi$. Suppose, for any edge (u', v') from the meta-bipartite graph formed for two layers, the assigned weights are in the same proportion across $\phi$s, i.e. $\frac{w(u', v')|\phi_A}{w(u', v')|\phi_D}$ = $c_1$, $\frac{w(u', v')|\phi_A}{w(u', v')|\phi_H}$ = $c_2$ and $\frac{w(u', v')|\phi_D}{w(u', v')|\phi_H}$ = $c_3$ for some constants $c_1$, $c_2$ and $c_3$. In this case, the maximum flow that can be obtained for different choices of $\phi$s will also change in the same ratio, i.e. $\frac{MaxFlow(\phi_A)}{MaxFlow(\phi_D)}$ = $c_1$, $\frac{MaxFlow(\phi_A)}{MaxFlow(\phi_H)}$ = $c_2$ and $\frac{MaxFlow(\phi_D)}{MaxFlow(\phi_H)}$ = $c_3$. Thus, the same set of community matches will be obtained for such a case across all $\phi$s. 
\end{proof}

\textbf{\textit{Lemma 1.2}}
\textit{If the communities in layers $G_i$ and $G_j$ are cliques and inter-layer interactions between two communities involve unique members, then a 2-community that is obtained from $\phi_A$ and $\phi_D$ will also be a 2-community using $\phi_H$.}
%\vspace{-10pt}
\begin{proof}
Suppose, community $C_i^1$ from $G_i$ got matched to $C_j^1$ out of k possible options, $C_j^1$, $C_j^2$, ..., $C_j^k$ from $G_j$ using $\phi_A$ and $\phi_D$. This means, $|L_{i,j}^{1,1}|$ = $max_{1 \le p \le k}|L_{i,j}^{1,p}|$ (condition for $\phi_A$) and $\frac{|L_{i,j}^{1,1}|}{|V_i^1|*|V_j^1|}$ = $max_{1 \le p \le k}|L_{i,j}^{1,p}|$ (condition for $\phi_D$). As the communities are cliques, therefore their densities are 1, which further means that every node is a hub in its community. Thus, $|H_i^1|$ = $|V_i^1|$ and $|H_j^1|$ = $|V_j^1|$, $|H_j^2|$ = $|V_j^2|$, ..., $|H_j^k|$ = $|V_j^k|$. Moreover, as unique community member pairs are involved in the interaction thus $|H_{i,j}^{1,1}|$ = $|L_{i,j}^{1,1}|$ = $|H_{j,i}^{1,1}|$, $|H_{i,j}^{1,2}|$ = $|L_{i,j}^{1,2}|$ = $|H_{j,i}^{2,1}|$, ..., $|H_{i,j}^{1,k}|$ = $|L_{i,j}^{1,k}|$ = $|H_{j,i}^{k,1}|$. Therefore, for $\phi_H$, the inter-layer meta edge weight between $C_i^1$ and $C_j^1$ will be the maximum among all the weights assigned for the inter-layer meta edges going from $C_i^1$. Thus, among the k community alternatives from $G_j$, the community $C_i^1$ will be matched to $C_j^1$ by the network flow algorithm as for any other matching the overall flow across the meta-bipartite graph will reduce and may even reduce the total number of matches.
\end{proof}



\begin{comment}



\begin{enumerate}
\item Why is it different in the presence of multiple entities (heterogeneous multilayer networks)?
\item Explain how finding community of the multiplex as a whole will hide a lot of information.
\item Explain through IMDB examples what are the \textit{different} interpretations of a community. Give scenarios.
\item Give the definition with respect to the bipartite based approach, as used in the paper
\end{enumerate}

\subsection{Maximal Matching Approach}
\begin{enumerate}
\item Explain how by using network flow as a subroutine the proposed types of communities be obtained.
\item Explain the modeling of the meta bipartite graph
\item Explain the need for different weighing schemes for finding different types of communities
\item Can we comment on the number of couplings? How to decide the upper bound?
\end{enumerate}

\subsection{Metrics Proposed}
\begin{enumerate}
\item Give reasons of having different weighting schemes are important. Say that these are just few and many more can be defined based on analysis requirement
\item Introduce the 3 classes of metrics that have been used in the paper
\end{enumerate}

\subsubsection{Cumulative Edge Interaction (Metric M(E))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsubsection{Dense Group Interaction (Metric M(D))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsubsection{Hub Interaction (Metric M(H))}

\begin{enumerate}
\item Which class of analysis will need such a metric?
\item Formulation of metric \begin{itemize}
\item Different components of the metric
\item Is the dependence of the components directly proportional or inversely proportional?
\item What will be the range of the metric? What does high or low value mean?
\end{itemize}
\item How will the output of using this metric be interpreted?
\item How will layer-wise communities or inter-layer edges effect the range of this metric?
\end{enumerate}

\subsection{Comparison between Metrics}

\begin{enumerate}
\item A given director community may get attached different actor communities based on metrics. 
\item Under what circumstances/conditions do the different metrics give different/same outputs. Can lemmas be stated?
\item From the analytical point of view what does it mean if some couplings comes up as an output using multiple metrics
\item Does ordering the outputs based on metric values give any additional inference? What if the same coupling has different levels of importance in different metrics?
\end{enumerate}
\end{comment}

==> texFiles/old-Experiments.tex <==
\section{Experimental Analysis}
\label{sec:experiments}

In this section, we present the results of our  analysis of  ~\ref{list:maximum-interaction} through ~\ref{list:We-cyclic3-madm} discussed in Section~\ref{sec:application-and-analysis} on the IMDb data set~\cite{data/type2/IMDb} modeled as a HeMLN. To recap, we have 3 layers,  Actor (layer A), Director (layer D), and Movies (layer M) and 3 inter-layer relationships (directs-actor, acts-in-a-movie, and directs-movies.) We start with the individual layer analysis and  continue with all the 6 analysis using the approach proposed in this paper and discuss their corroboration with the intuitive expectations and analysis discussed earlier. 
%based on the k-community generated for the as described in Section \ref{sec:customize-maxflow}. 

%%\abhi{2/28/2019}{Added a line about how Infomap works}
\textbf{Experiment Setup:} A random set of 1000 movies that released anywhere in the world in the period from 2001 to 2015 were chosen for building the HeMLN, comprising of %2\% of the total (244565) actors and 1\% of the total (93085) directors
4588 actors and 1091 directors from that period. A 1-community is computed for each layer using the widely used package Infomap~\cite{InfoMap2014}, that works in a hierarchical fashion while optimizing the \textit{map equation}, which exploits the \textit{information - theoretic duality} between the problem of compressing data, and the problem of detecting and extracting significant patterns or structures (communities) within those data based on \textit{information flow}. % and Louvain~\cite{DBLP:Louvain}. 
We use the publicly available package from NetworkX for the bipartite graph match~\cite{Python:maximal-match}. The k-community detection Algorithm \ref{alg:k-community} was implemented in Python version 3.6 and was executed on a quad-core $8^{th}$ generation Intel i5 processor Windows 10 machine with 8 GB RAM. 


\subsection{IMD\MakeLowercase{b} Individual Layer Analysis}

For the purposes of this analysis, we generated disjoint 1-community for each individual layer.
%with a setting which assigns any node to at most one community (i.e. computes disjoint communities). Infomap works in a hierarchical fashion while optimizing the \textit{map equation}, which exploits the \textit{information-theoretic duality} between the problem of compressing data, and the problem of detecting and extracting significant patterns or structures (communities) within those data based on \textit{information flow}. 
The statistics for each layer are shown in Table~\ref{table:layer-stats}. The community size distribution is shown as a cloud for each layer in Figure~\ref{fig:cloud}.
%For Layer A, Layer D (Director) and Layer M (Movie), the number of communities (with more than one vertex) detected were 862, 18 and 5, respectively. 
%%For each layer, 1-community is numbered starting from 1. 
%These 1-community have been used to generate the other k-community, as per analysis requirement. 
For clarity, we show each layer with layer prefix and community id.   %from total matches obtained, i.e. the partial matches and inter-layer edge have not been listed. Figure~\ref{fig:cloud} shows each layer as a cloud for understanding the size distribution of communities.

\begin{figure}[h]
   \centering \includegraphics[width=\linewidth]{./figures/cloud-v2}
   %\caption{Word Cloud showing the relative sizes of different actor (\textbf{Ai}s), directors (\textbf{Di}s) and movie (\textbf{Mi}s) communities}
   \caption{Community Clouds Based on Size}
   \label{fig:cloud}
%\vspace{-10pt}
\end{figure}


A number of insights can be gleaned from layer analysis. The average, mode and median actor community size are 5.3, 4 and 4, respectively. The proportion of communities of median size or less (529 out of 819 or at least 61\%) indicate that co-acting is limited to smaller groups of actors. There is only 1 large group (51) of co-actors. Further, 790 (92\%) clique communities indicate that actors who co-act do it with the same group.  In contrast,  the number of communities is proportionately less (with respect to the number of nodes) in the director layer indicating that directors do not limit themselves to directing a small set of genres. The lower number of communities in the Movie (rating) layer is expected as it is a layer of 5 non-overlapping rating ranges.  Also, 35\% of movies (major chunk) have ratings in the range [6-8), A small number of movies (community M5) has the lowest range of rating [0, 2). Also, we know that all of them are cliques.

%%Moreover, from the director communities it can be deduced that over the world, there are primarily 18 diverse types of directors based on the diversity of movie genres they direct.  The 1-community for each layer is - Layer A: \{$c_A^1$, $c_A^2$, ..., $c_A^{881}$\}, Layer D: \{$c_D^1$, $c_D^2$, ..., $c_D^{18}$\} and Layer M: \{$c_M^1$, $c_M^2$, ..., $c_M^{5}$\}.

\begin{table}[h!t]
\centering
    \begin{tabular}{|c|c|c|c|}
            \hline
                 & Actor & Director & Movie \\
            \hline
                \#Vertices & 4588 & 1091 & 1000 \\
%            Layer Density & 10255 & 91991 & 87492 \\
            \hline
            Layer Density & 0.00097 & 0.15471 & 0.17516 \\
            \hline
            \#Comm. (Size $>$ 1) & 862 & 18 & 5 \\
            \hline
                \#Clique Communities & 790 & 7 & 5 \\
            \hline
                \% Vertices in Cliques & 82.6\% & 7.4\% &  100\%\\
            \hline
                Avg. Size & 5.3 & 60.61 & 132.5 \\                
            \hline
                Mode Size (\#Comm) & 4 (510) & 2 (3) & - \\
            \hline
                Median Size (\#Comm.) & 4 (510) & 31.5 (0) & 57 (0)\\
            \hline
                Max. Size (\#Comm.) & 51 (1) & 357 (1) & 352 (1)\\
            \hline
                Min. Size (\#Comm.) & 2 (19) & 2 (3) & 3 (1)\\
            \hline

        \end{tabular}
            \caption{1-community Statistics for IMDb HeMLN}
    \label{table:layer-stats}
\end{table}



%%\textcolor{blue}{SB: I guess the other actor communities not shown in the table did not get maximal matching. Maybe we should clearly write that. All the actor communities that got matched are with non-famous people who did 1-2 movies. Also Abhishek--do you know any of the genres associated with the director communities ? Let me know}
\subsection{IMD\MakeLowercase{b} 2-community Analysis}
\label{sec:2-com}

%The evaluation of any analysis is a two-fold process that have been experimentally illustrated using the ones listed in Section \ref{sec:customize-maxflow}.

%\noindent\textbf{Mapping of Requirements to 2-community Specification:} Based on the requirements, each analysis from \ref{list:maximum-interaction} to \ref{list:hub-participation}, needs to obtain 2-community using the Layer A (Actor) and Layer D (Director). Thus, the required 2-community specification is A $\Theta_{A,D}$ D. However, every analysis requires a different metric for pairing the communities from A and D, which are $\omega_e$ for \ref{list:maximum-interaction}, $\omega_d$ for \ref{list:density} and $\omega_h$ for \ref{list:hub-participation} (as discussed in Section \ref{sec:customize-maxflow}. 

%\noindent\textbf{Map Requirements to 2-community Specification:} Based on the requirements, Analysis \ref{list:maximum-interaction} to \ref{list:hub-participation}, need to obtain 2-community using the Layer A (Actor) and Layer D (Director). Thus, the required 2-community specification is A $\Theta_{A,D}$ D. However, every analysis requires a different metric for pairing the communities from A and D, which are $\omega_e$ for \ref{list:maximum-interaction}, $\omega_d$ for \ref{list:density} and $\omega_h$ for \ref{list:hub-participation} (as discussed in Section \ref{sec:customize-maxflow}. These three analysis the base case of the k-community definition.


\begin{table}[h!t]
\renewcommand{\arraystretch}{1}
\centering
\subfloat[]{

    \begin{tabular}{|p{0.95cm}|p{0.75cm}|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:maximum-interaction}}, $\omega_e$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        A6 & D1 \\
        \hline
        A252 & D2 \\
        \hline
        \textcolor{applegreen}{\textbf{A577}:c} & \textcolor{applegreen}{\textbf{D3}} \\
        \hline
        A2 & D4 \\
        \hline
        \textcolor{applegreen}{\textbf{A555}:c} & \textcolor{applegreen}{\textbf{D5}} \\
        \hline
        A100:c & D6 \\
        \hline
        \textcolor{applegreen}{\textbf{A374}:c} & \textcolor{applegreen}{\textbf{D7}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A484}:c} & \textcolor{applegreen}{\textbf{D8}} \\
        \hline
        A10 & D9 \\
        \hline
        A683:c & D10 \\
        \hline
        \textcolor{applegreen}{\textbf{A83}:c} & \textcolor{applegreen}{\textbf{D11}} \\
        \hline
        \textcolor{applegreen}{\textbf{A89}:c} & \textcolor{applegreen}{\textbf{D12}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A46}:c} & \textcolor{applegreen}{\textbf{D13}:c} \\
        \hline
        A161:c & D14:c \\
        \hline
        \textcolor{applegreen}{\textbf{A220}:c} & \textcolor{applegreen}{\textbf{D15}} \\
        \hline
        A85:c & D16:c \\
        \hline
        A188 & D17:c \\
        \hline
        A53:c & D18:c \\
        \hline
        \end{tabular}
        \label{table:A1-results-allD}
}
%\qquad
\subfloat[]{

    \begin{tabular}{|p{0.95cm}|p{0.75cm}|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:density}}, $\omega_d$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        A511:c & D1 \\
        \hline
        A204:c & D2 \\
        \hline
        \textcolor{applegreen}{\textbf{A577}:c} & \textcolor{applegreen}{\textbf{D3}} \\
        \hline
        A483:c & D4 \\
        \hline
        \textcolor{applegreen}{\textbf{A555}:c} & \textcolor{applegreen}{\textbf{D5}} \\
        \hline
        A332:c & D6 \\
        \hline
        \textcolor{applegreen}{\textbf{A374}:c} & \textcolor{applegreen}{\textbf{D7}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A484}:c} & \textcolor{applegreen}{\textbf{D8}} \\
        \hline
        A158:c & D9 \\
        \hline
        A683:c & D10 \\
        \hline
        \textcolor{applegreen}{\textbf{A83}:c} & \textcolor{applegreen}{\textbf{D11}} \\
        \hline
        \textcolor{applegreen}{\textbf{A89}:c} & \textcolor{applegreen}{\textbf{D12}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A46}:c} & \textcolor{applegreen}{\textbf{D13}:c} \\
        \hline
        A824:c & D14:c \\
        \hline
        \textcolor{applegreen}{\textbf{A220}:c} & \textcolor{applegreen}{\textbf{D15}} \\
        \hline
        A310:c & D16:c \\
        \hline
        A330:c & D17:c \\
        \hline
        A793:c & D18:c \\
        \hline
        \end{tabular}
        \label{table:A2-results-allD}
}
%\qquad
%\vspace{-1pt}
\subfloat[]{
    \begin{tabular}{|p{0.95cm}|p{0.75cm}|}
        \hline
         \multicolumn{2}{|c|}{\textbf{\ref{list:hub-participation}}, $\omega_h$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        A511:c & D1 \\
        \hline
        A204:c & D2 \\
        \hline
        \textcolor{applegreen}{\textbf{A577}:c} & \textcolor{applegreen}{\textbf{D3}} \\
        \hline
        A483:c & D4 \\
        \hline
        \textcolor{applegreen}{\textbf{A555}:c} & \textcolor{applegreen}{\textbf{D5}} \\
        \hline
        A332:c & D6 \\
        \hline
        \textcolor{applegreen}{\textbf{A374}:c} & \textcolor{applegreen}{\textbf{D7}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A484}:c} & \textcolor{applegreen}{\textbf{D8}} \\
        \hline
        A381:c & D9 \\
        \hline
        A828:c & D10 \\
        \hline
        \textcolor{applegreen}{\textbf{A83}:c} & \textcolor{applegreen}{\textbf{D11}} \\
        \hline
        \textcolor{applegreen}{\textbf{A89}:c} & \textcolor{applegreen}{\textbf{D12}:c} \\
        \hline
        \textcolor{applegreen}{\textbf{A46}:c} & \textcolor{applegreen}{\textbf{D13}:c} \\
        \hline
        A824:c & D14:c \\
        \hline
        \textcolor{applegreen}{\textbf{A220}:c} & \textcolor{applegreen}{\textbf{D15}} \\
        \hline
        A310:c & D16:c \\
        \hline
        A330:c & D17:c \\
        \hline
        A793:c & D18:c \\
        \hline        
        \end{tabular}

        \label{table:A3-results-allD}
}
\vspace{-8pt}
\caption*{\textbf{All Communities}, c indicates a clique,  \textcolor{applegreen}{44.4\% common pairings} (862 A Communities, 18 D Communities)}

\subfloat[]{

    \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:maximum-interaction}}, $\omega_e$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        \textcolor{blue}{\textbf{A374}} & \textcolor{blue}{\textbf{D7}} \\
        \hline
        \textcolor{blue}{\textbf{A89}} & \textcolor{blue}{\textbf{D12}} \\
        \hline
        \textcolor{blue}{\textbf{A46}} & \textcolor{blue}{\textbf{D13}} \\
        \hline
        A161 & D14 \\
        \hline
        A85 & D16 \\
        \hline
        \textcolor{blue}{\textbf{A330}} & \textcolor{blue}{\textbf{D17}} \\
        \hline
        A53 & D18 \\
        \hline
        \end{tabular}
        \label{table:A1-results-Deq1}
}
%\qquad
\subfloat[]{

    \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:density}}, $\omega_d$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        \textcolor{blue}{\textbf{A374}} & \textcolor{blue}{\textbf{D7}} \\
        \hline
        \textcolor{blue}{\textbf{A89}} & \textcolor{blue}{\textbf{D12}} \\
        \hline
        \textcolor{blue}{\textbf{A46}} & \textcolor{blue}{\textbf{D13}} \\
        \hline
        A824 & D14 \\
        \hline
        A310 & D16 \\
        \hline
        \textcolor{blue}{\textbf{A330}} & \textcolor{blue}{\textbf{D17}} \\
        \hline
        A793 & D18 \\
        \hline
        \end{tabular}
        \label{table:A2-results-Deq1}
}
%\qquad
\subfloat[]{
    \begin{tabular}{|c|c|}
        \hline
         \multicolumn{2}{|c|}{\textbf{\ref{list:hub-participation}}, $\omega_h$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        \textcolor{blue}{\textbf{A374}} & \textcolor{blue}{\textbf{D7}} \\
        \hline
        \textcolor{blue}{\textbf{A89}} & \textcolor{blue}{\textbf{D12}} \\
        \hline
        \textcolor{blue}{\textbf{A46}} & \textcolor{blue}{\textbf{D13}} \\
        \hline
        A824 & D14 \\
        \hline
        A310 & D16 \\
        \hline
        \textcolor{blue}{\textbf{A330}} & \textcolor{blue}{\textbf{D17}} \\
        \hline
        A793 & D18 \\
          \hline
        \end{tabular}

        \label{table:A3-results-Deq1}
}
\vspace{-8pt}
\caption*{\textbf{Clique Communities only}, \textcolor{blue}{57.14\% common pairings} (790 A Communities, 7 D Communities)}

\subfloat[]{

    \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:maximum-interaction}}, $\omega_e$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        A6 & D1 \\
        \hline
        \textcolor{cyan}{\textbf{A252}} & \textcolor{cyan}{\textbf{D2}} \\
        \hline
        A1 & D3 \\
        \hline
        A2 & D4 \\
        \hline
        A187 & D6 \\
        \hline
        A4 & D8 \\
        \hline
        A10 & D9 \\
        \hline
        A17 & D11 \\
        \hline
        A129 & D15 \\
        \hline
        \end{tabular}
        \label{table:A1-results-Dlt1}
}
%\qquad
\subfloat[]{

    \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{\textbf{\ref{list:density}}, $\omega_d$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
         A59 & D1 \\
        \hline
         \textcolor{cyan}{\textbf{A252}} & \textcolor{cyan}{\textbf{D2}} \\
        \hline
         A257 & D3 \\
        \hline
         A190 & D4 \\
        \hline
         A293 & D6 \\
        \hline
         A246 & D8 \\
        \hline
         A10 & D9 \\
        \hline
         A122 & D11 \\
        \hline
         A129 & D15 \\
        \hline
        \end{tabular}
        \label{table:A2-results-Dlt1}
}
%\qquad
\subfloat[]{
    \begin{tabular}{|c|c|}
        \hline
         \multicolumn{2}{|c|}{\textbf{\ref{list:hub-participation}}, $\omega_h$} \\
        \hline
        $c_A$ & $c_D$ \\
        \hline
        A59 & D1 \\
        \hline
         \textcolor{cyan}{\textbf{A252}} & \textcolor{cyan}{\textbf{D2}} \\
        \hline
        A184 & D3 \\
        \hline
        A190 & D4 \\
        \hline
        A293 & D6 \\
        \hline
        A4 & D8 \\
        \hline
        A16 & D9 \\
        \hline
        A122 & D11 \\
        \hline
        \end{tabular}

        \label{table:A3-results-Dlt1}
}
\vspace{-8pt}
\caption*{\textbf{Non-clique Communities only}, \textcolor{cyan}{11.11\% common pairings} (72 A Communities, 11 D Communities)}

\caption{2-community results for (A $\Theta_{A,D}$ D)}
\label{table:2-community}
\vspace{-10pt}
    
\end{table}


With 3 layers and 3 weight metrics, there are a total of 9 possible 2-community specifications. As the movie-rating layer has very few (and only clique) communities, we have chosen the A and D layers (with A as the left set of the bipartite match) for analysis using different metrics as shown in ~\ref{list:maximum-interaction} to ~\ref{list:hub-participation}. As each metric is based on a different intuition  for inter-layer coupling, they are expected to give different results.

%%\noindent\textbf{Analysis Results: } %Table
%\ref{table:2-community} shows the results as community pairings for the chosen metric. %In addition to the matched communities, 2-community also contains the corresponding bipartite graph (i.e. $x_{A,D}$s) that have not been shown here.
Table \ref{table:A1-results-allD}, \ref{table:A2-results-allD}, and \ref{table:A3-results-allD} show the results of 2-community as community pairings, respectively, for each metric.
When the entire 1-community  is used for each layer,  \textbf{44.4\% pairings (8 out of the 18) (marked in \textcolor{applegreen}{green})} are the \textit{same across metrics}. In all the common pairings, at least one of the participating community is a clique. % As is shown in Lemma ?, this is the case when communities are cliques. We have verified that all  7 cliques of D result in the same pairings across $\omega$.

To understand the analysis differences across $\omega$, we grouped non-clique (density $<$ 1) communities from each layer for analysis.
Table \ref{table:A1-results-Dlt1}-\ref{table:A3-results-Dlt1}
shows the results for non-clique communities from each layer.
Just \textbf{one common pairing} is found (marked in \textcolor{cyan}{\textbf{cyan}}) \textbf{validating the uniqueness of proposed  metrics.}

For completeness, Table \ref{table:A1-results-Deq1}, \ref{table:A2-results-Deq1}, and \ref{table:A3-results-Deq1} show the community pairings when only cliques are used from each layer. Every matched pair that appears for $\omega_e$ (Table \ref{table:A1-results-Deq1}) and $\omega_d$ (Table \ref{table:A2-results-Deq1}) satisfied the conditions listed in Lemma \ref{lemma:edToh}, thus justifying their appearance for $\omega_h$ (Table \ref{table:A3-results-Deq1}) as well (marked in \textcolor{blue}{\textbf{blue}}.)

\begin{comment}

used to create the community bipartite graph to obtain the matches. %The number of matches for a specification is limited by the layer having the lower number of tuples in 1-community, i.e. the director layer.
The number of pairings is 18 for the three analysis (or metrics), as the director layer with lower number of communities acts as the bounding layer. It can be observed that 44.4\% pairings (8 out of the 18) (marked in \textcolor{applegreen}{green}) are common across all metrics. On closer look, it was noticed that for each common pairing \textit{at least one of the communities was a clique}. Thus, it can be claimed that \textit{in the presence of cliques, a large number of pairings that are common to all metrics} will be produced. In order to justify this claim, we repeated the 2-community generation for two different cases - one with clique communities (density = 1) and another with non-clique communities (density $<$ 1).    

 Whereas, for the case where non-clique communities are considered from both layers just one common pairing is found (marked in \textcolor{cyan}{\textbf{cyan}} in Table \ref{table:A1-results-Dlt1}-\ref{table:A3-results-Dlt1}). Thus, justifying that when the community densities \textit{vary}, \textbf{a given community from one of the layers \textit{can} pair with \textit{different communities} from the other layer based on metric chosen giving rise to diverse insights}. 

\end{comment}
%% Table 2g,h,i figure commented out

\begin{comment}


\begin{figure}[ht]
   \centering \includegraphics[width=0.8\linewidth]{./figures/noncliques_ad}
   \caption{2-community results (community matches) for (A $\Theta_{A,D}$ D) with only non-clique communities with metric \textcolor{applegreen}{$\omega_e$ (Analysis \ref{list:maximum-interaction})}, \textcolor{violet}{$\omega_d$ (Analysis \ref{list:density})} and \textcolor{cyan}{$\omega_h$ (Analysis \ref{list:hub-participation})}}
   \label{fig:noncliques-ad}
%\vspace{-10pt}
\end{figure}

\end{comment}

We know that the metric $\omega_e$ does not depend on the community characteristics, such as density and hub participation, unlike $\omega_d$ and $\omega_h$. This can also be validated from the results. All the actor communities that are part of matches for $\omega_d$ (Table \ref{table:A2-results-allD}) and $\omega_h$ (Table \ref{table:A3-results-allD}) are cliques, marked by \textit{`c'}, (which should be the case.) However, for the Table~\ref{table:A1-results-allD} which uses $\omega_e$, it is not the case validating our intuition. Even the removal of cliques does not effect the non-clique matches that were obtained for $\omega_e$ (Table \ref{table:A1-results-allD} and Table \ref{table:A1-results-Dlt1}.) 

%%Further, if a community is a clique then the chances of it appearing in a matching are more w.r.t the metrics $\omega_d$ (density = 1) and $\omega_h$ (every participating node is a hub). This cannot be said for the metric $\omega_e$, as it depends solely on the number of inter-layer edges. This can also be seen in the results where Thus, \textbf{presence of cliques effect $\omega_d$ and $\omega_h$ more as compared to $\omega_e$}.

\begin{comment}


\noindent\textbf{Observations from Results:} Few observations made from the 2-community results obtained.

\begin{itemize}
    \item Tim Burton (director of Alice in Wonderland, Planet of the Apes, Dumbo etc.) belongs to similar genre-based director community 3, which is paired with co-actor community 1 that has Indian actor Salman Khan as one of the members (metric $\omega_e$), co-actor community 257 that has Tim Theron as a member (metric $\omega_d$) and co-actor community 184 that has Egyptian actor Lamia El Amir as a member (metric $\omega_h$). These pairings illustrate how directors and actors from across the world can be grouped based on different similarity requirements.
    \item talk about how clique communities effect the metrics (e independent, d and h are dependent). subtract first column and comment on it.
    \item draw a diagram to illustrate the meaning of different pairings. give one or two examples about how a director community with different region distributions can get paired with different actor communities
    
\end{itemize}

\end{comment}

\begin{comment}


\begin{table}[h!t]
\renewcommand{\arraystretch}{1.4}
\centering

    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{\ref{list:maximum-interaction}} & \textbf{\ref{list:density}} &  \textbf{\ref{list:hub-participation}} \\
        \hline
        (A $\Theta_{A,D}$ D), $\omega_e$ & (A $\Theta_{A,D}$ D), $\omega_d$ &  (A $\Theta_{A,D}$ D), $\omega_h$ \\
        \hline
        \hline
        $<c_A^1, c_D^3 ; x_{A,D}>$ & $<c_A^{10}, c_D^9 ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^6, c_D^1 ; x_{A,D}>$ & $<c_A^{129}, c_D^{15} ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^4, c_D^8 ; x_{A,D}>$ & $<c_A^{59}, c_D^1 ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^2, c_D^4 ; x_{A,D}>$ & $<c_A^{122}, c_D^{11} ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^{17}, c_D^{11} ; x_{A,D}>$ & $<c_A^{190}, c_D^{4} ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^{10}, c_D^9 ; x_{A,D}>$ & $<c_A^{252}, c_D^{2} ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^{129}, c_D^{15} ; x_{A,D}>$ & $<c_A^{257}, c_D^{3} ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        $<c_A^{187}, c_D^6 ; x_{A,D}>$ & $<c_A^{246}, c_D^8 ; x_{A,D}>$ & \\
        \hline
        $<c_A^{252}, c_D^2 ; x_{A,D}>$ & $<c_A^{293}, c_D^6 ; x_{A,D}>$ & $<c_A^, c_D^ ; x_{A,D}>$ \\
        \hline
        \end{tabular}
            \caption{2-community specification and results for Analysis in Section \ref{sec:customize-maxflow} (community density $\neq$ 1)}
    \label{table:layer-stats}
    
\end{table}



\begin{table}[h!t]
\renewcommand{\arraystretch}{1.4}
\centering
\subfloat[Analysis \ref{list:maximum-interaction}]{

    \begin{tabular}{|c|}
        \hline
        \textbf{\ref{list:maximum-interaction}} \\
        \hline
        (A $\Theta_{A,D}$ D), $\omega_e$ \\
        \hline
        \hline
        $<c_A^1, c_D^3 ; x_{A,D}>$ \\
        \hline
        $<c_A^6, c_D^1 ; x_{A,D}>$ \\
        \hline
        $<c_A^4, c_D^8 ; x_{A,D}>$ \\
        \hline
        $<c_A^2, c_D^4 ; x_{A,D}>$ \\
        \hline
        $<c_A^{17}, c_D^{11} ; x_{A,D}>$ \\
        \hline
        $<c_A^{10}, c_D^9 ; x_{A,D}>$ \\
        \hline
        $<c_A^{129}, c_D^{15} ; x_{A,D}>$ \\
        \hline
        $<c_A^{187}, c_D^6 ; x_{A,D}>$ \\
        \hline
        $<c_A^{252}, c_D^2 ; x_{A,D}>$ \\
        \hline
        \end{tabular}
        \label{table:A1-results}
}
\qquad
\subfloat[Analysis \ref{list:density}]{

    \begin{tabular}{|c|}
        \hline
        \textbf{\ref{list:density}} \\
        \hline
        (A $\Theta_{A,D}$ D), $\omega_d$ \\
        \hline
        \hline
         $<c_A^{10}, c_D^9 ; x_{A,D}>$ \\
        \hline
         $<c_A^{129}, c_D^{15} ; x_{A,D}>$ \\
        \hline
         $<c_A^{59}, c_D^1 ; x_{A,D}>$ \\
        \hline
         $<c_A^{122}, c_D^{11} ; x_{A,D}>$ \\
        \hline
         $<c_A^{190}, c_D^{4} ; x_{A,D}>$ \\
        \hline
         $<c_A^{252}, c_D^{2} ; x_{A,D}>$ \\
        \hline
         $<c_A^{257}, c_D^{3} ; x_{A,D}>$ \\
        \hline
         $<c_A^{246}, c_D^8 ; x_{A,D}>$ \\
        \hline
         $<c_A^{293}, c_D^6 ; x_{A,D}>$ \\
        \hline
        \end{tabular}
        \label{table:A2-results}
}
\qquad
\subfloat[Analysis \ref{list:hub-participation}]{
    \begin{tabular}{|c|c|c|}
        \hline
         \textbf{\ref{list:hub-participation}} \\
        \hline
        (A $\Theta_{A,D}$ D), $\omega_h$ \\
        \hline
        \hline
        $<c_A^4, c_D^8 ; x_{A,D}>$ \\
        \hline
         $<c_A^{16}, c_D^9 ; x_{A,D}>$ \\
        \hline
        $<c_A^{59}, c_D^1 ; x_{A,D}>$ \\
        \hline
        $<c_A^{122}, c_D^{11} ; x_{A,D}>$ \\
        \hline
        $<c_A^{184}, c_D^3 ; x_{A,D}>$ \\
        \hline
        $<c_A^{190}, c_D^4 ; x_{A,D}>$ \\
        \hline
        $<c_A^{252}, c_D^2 ; x_{A,D}>$ \\
        \hline
        $<c_A^{293}, c_D^6 ; x_{A,D}>$ \\
        \hline
        \end{tabular}

        \label{table:A3-results}
}
\caption{2-community specification and results for Analysis in Section \ref{sec:customize-maxflow} (community density $\neq$ 1)}
\label{table:2-community}
    
\end{table}

\end{comment}




\subsection{IMD\MakeLowercase{b} Acyclic 3-community Analysis}
%choose any one metric that gives minimum overlap across different 3-community sequences. this can be repeated for 3-community (with cycle) sequences

%\noindent\textbf{Map Requirements to Acyclic 3-community Specification:}
For \ref{list:We-acyclic3-adm} and \ref{list:We-acyclic3-mad}, we need to generate \textit{acyclic} 3-community based on the specification which also includes order and metric $\omega_e$.
%look into \textit{how communities from two layers interact with the communities of a third (central) layer}. %needs to group the  actor and movie communities with a director community. Thus,
Specifically, for analysis \ref{list:We-acyclic3-adm} and ~\ref{list:We-acyclic3-mad},
the director and actor layer, become the left layer for community bipartite graph, respectively, during the second composition.
%based on   specifications - A $\Theta_{A,D}$ D $\Theta_{D,M}$ M; $\omega_e$ (for Analysis \ref{list:We-acyclic3-adm}) and   M $\Theta_{M,A}$ A $\Theta_{A,D}$ D; $\omega_e$ (for Analysis \ref{list:We-acyclic3-mad}).

%The multilayer structure of the tuples in 3-community will be \textit{acyclic} in nature. Additionally, both analysis need to pair communities such that \textit{the inter-layer interaction is maximized}, as the chosen metric is  $\omega_e$. 

%Both these analysis fall under case (i) of the recursive case, where the right layer has not been seen earlier. %These mappings illustrate that for given k layers (3 in this case), different specifications are possible (and meaningful) based on the analysis requirements.

\begin{comment}



\begin{table}[h!t]
\renewcommand{\arraystretch}{1}
\centering
\subfloat[]{

    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{\textbf{\ref{list:We-acyclic3-adm}}, $\omega_e$} \\
        \hline
        \multicolumn{3}{|c|}{\textbf{A $\Theta_{A,D}$ D $\Theta_{D,M}$ M}} \\
        \hline
        $c_A$ & $c_D$ & $c_M$\\
        \hline
         A6 & D1 & M1\\
        \hline
         A252 & D2 & M2\\
        \hline
         A2 & D4 & M4\\        
        \hline
         A555 & D5 & M3\\
        \hline
         A100 & D6 & M5\\
        \hline
         \multicolumn{3}{|c|}{13 Partial Matches (on M)} \\
         \hline
        \end{tabular}
        \label{table:A4-results-allD}
}
%\qquad
\subfloat[]{
    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{\textbf{\ref{list:We-acyclic3-amd}}, $\omega_e$} \\
        \hline
        \multicolumn{3}{|c|}{\textbf{A $\Theta_{A,M}$ M $\Theta_{M,D}$ D}} \\
        \hline        
        $c_A$ & $c_M$ & $c_D$\\
        \hline
         A60 & M1 & D1\\
        \hline
         A2 & M2 & D2\\
        \hline
         A36 & M3 & D5\\
        \hline
         A1 & M4 & D4\\
        \hline
         A276 & M5 & D6\\
        \hline
         \multicolumn{3}{|c|}{0 Partial Matches (on D)} \\
         \hline
        \end{tabular}

        \label{table:A5-results-allD}
}
\caption{Acyclic 3-community results (Only Total Matches Shown with Community Ids)}
\label{table:3-community}
    
\end{table}

\end{comment}

\begin{figure}[ht]
   \centering \includegraphics[width=\linewidth]{./figures/A4-adm-v2}
   \caption{Acyclic 3-community (\textbf{total and partial})}
   \label{fig:A4-adm}
%\vspace{-10pt}
\end{figure}


Figures~\ref{fig:A4-adm} and ~\ref{fig:A5-mad}  show the 3-community analysis results diagrammatically for \ref{list:We-acyclic3-adm} and \ref{list:We-acyclic3-mad}, respectively. %The figures also show the matches during each iteration using colored lines between communities. %\textcolor{blue}{Blue} lines indicate \textbf{pair-wise matches} for each composition. \textcolor{blue}{Broken blue} indicates \textbf{partial matches} along a
% revie total and partial
%path. \textcolor{blue}{\textbf{Bold blue}} indicates matching pairs for the \textbf{complete analysis}.
For analysis \ref{list:We-acyclic3-adm}, 18 elements (consistent matches) are obtained after the first composition, bounded by the 18 communities in the director layer. For the second composition, although all the 18 communities from layer director are carried over (as they paired during base case), only 5 %will match as there are only 5 communities
produce consistent matches with the movie layer, to get extended to become total elements (\textcolor{blue}{\textbf{bold blue line}}), whereas, for the other 13 there was a no match (\textcolor{blue}{broken blue lines}), thus becoming partial elements. %That is, those actor-director community pairings that \textbf{did not find a match} with a movie community.
Similarly, for \ref{list:We-acyclic3-mad}, every pairing from the first composition got extended in the second composition to produce 5 total elements (\textcolor{blue}{\textbf{bold blue lines}}), bounded by movie communities.  Moreover, for both the  result sets, none of the total elements overlap. Thus, \textbf{the \textit{order}} in which k layers are specified to obtain k-community determines the set of partial and total elements, providing insights corresponding to analysis specification.



\begin{figure}[ht]
   \centering \includegraphics[width=\linewidth]{./figures/A5-mad-v2}
   \caption{Acyclic 3-community (\textbf{no partial elements})}
   \label{fig:A5-mad}
\vspace{-10pt}
\end{figure}


\begin{comment}


\begin{table}[h!t]
\renewcommand{\arraystretch}{1}
\centering
\subfloat[]{

    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multicolumn{5}{|c|}{\textbf{\ref{list:We-acyclic3-1}}, $\omega_e$} \\
        \hline
        \multicolumn{5}{|c|}{\textbf{A $\Theta_{A,D}$ D $\Theta_{D,M}$ M}} \\
        \hline
        $c_A$ & $c_D$ & $c_M$ & $x_{A,D}$ & $x_{D,M}$\\
        \hline
         6 & 1 & 1 & &\\
        \hline
         252 & 2 & 2 & &\\
        \hline
        577 & 3 & 0 & & $\phi$ \\
        \hline
         2 & 4 & 4 & &\\        
        \hline
         555 & 5 & 3 & &\\
        \hline
         100 & 6 & 5 & &\\
        \hline
        374 & 7 & 0 & & $\phi$ \\
        \hline
        484 & 8 & 0 & & $\phi$ \\
        \hline
        10 & 9 & 0 & & $\phi$ \\
        \hline
        683 & 10 & 0 & & $\phi$ \\
        \hline
        83 & 11 & 0 & & $\phi$ \\
        \hline
        89 & 12 & 0 & & $\phi$ \\
        \hline
        46 & 13 & 0 & & $\phi$ \\
        \hline
        161 & 14 & 0 & & $\phi$ \\
        \hline
        220 & 15 & 0 & & $\phi$ \\
        \hline
        85 & 16 & 0 & & $\phi$ \\
        \hline
        188 & 17 & 0 & & $\phi$ \\
        \hline
        53 & 18 & 0 & & $\phi$ \\
        \hline
        \end{tabular}
        \label{table:A4-results-allD}
}
\qquad
\subfloat[]{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multicolumn{5}{|c|}{\textbf{\ref{list:We-acyclic3-2}}, $\omega_e$} \\
        \hline
        \multicolumn{5}{|c|}{\textbf{A $\Theta_{A,M}$ M $\Theta_{M,D}$ D}} \\
        \hline        
        $c_A$ & $c_M$ & $c_D$ & $x_{A,M}$ & $x_{M,D}$\\
        \hline
         60 & 1 & 1 & &\\
        \hline
         2 & 2 & 2 & &\\
        \hline
         36 & 3 & 5 & &\\
        \hline
         1 & 4 & 4 & &\\
        \hline
         276 & 5 & 6 & &\\
        \hline
        \end{tabular}

        \label{table:A5-results-allD}
}
\caption{Acyclic 3-community results}
\label{table:3-community}
    
\end{table}

\end{comment}





\subsection{IMD\MakeLowercase{b} Cyclic 3-community Analysis}

Since 6 analysis orderings are possible for 3 layers and 3 sets of bipartite graphs forming a cycle (18 if metrics are included), choosing the order is important. \ref{list:We-cyclic3-madm} uses one of those orderings (M $\Theta_{M,A}$ A $\Theta_{A,D}$ D $\Theta_{D,M}$ M; $\omega_e$) where actors who are coupled with movie ratings collectively are further coupled with directors (giving directors who direct the popular actors for each rating.) This is coupled again with movies to check back whether the same director groups also have similar ratings. We have chosen $\omega_e$ for coupling. 

%\noindent\textbf{Map Requirements to Cyclic 3-community Specification:} %In case of analysis \ref{list:We-cyclic3-adma}, we need to find out the movie rating communities that have maximum interaction with the paired actor and director communities. Thus, in this analysis the required output will be a group of 3 community ids (one from each layer) where every pair has strong interaction between them. Thus, the structure of the results will be a cyclic 3-community. The specification for this analysis will be - A $\Theta_{A,D}$ D $\Theta_{D,M}$ M $\Theta_{M,A}$ A with chosen metric being, $\omega_e$.
%In analysis \ref{list:We-cyclic3-adma}, we need to find out the movie rating communities that have \textit{maximum interaction} with the paired actor and director communities. Here the expected total matches will be groups of 3 community ids (one from each layer) where every pair has strong interaction between them. Thus, the structure of the total matches will be a \textit{cyclic 3-community}. The specification for this analysis will be - A $\Theta_{A,D}$ D $\Theta_{D,M}$ M $\Theta_{M,A}$ A with chosen metric being, $\omega_e$.
%%In analysis \ref{list:We-cyclic3-madm}, we need to find out whether the director communities that have \textit{maximum interaction} with the \textit{most popular} actor communities w.r.t. each movie rating communities are also \textit{most popular} w.r.t to the same movie rating community. Here the expected total matches will be groups of 3 community ids (one from each layer) where every pair has strong interaction between them. Thus, the structure of the \textit{total} matches will be a \textit{cyclic 3-community}. The specification for this analysis will be - M $\Theta_{M,A}$ A $\Theta_{A,D}$ D $\Theta_{D,M}$ M with chosen metric being, $\omega_e$.


\begin{comment}


\begin{table}[h!t]
\renewcommand{\arraystretch}{1}
\centering
\subfloat[\textit{Final Iteration}]{

    \begin{tabular}{|c|c|c|c|}
        \hline
        \multicolumn{4}{|c|}{\textbf{\ref{list:We-cyclic3-madm}}, $\omega_e$} \\
 %       \hline
%        \multicolumn{4}{|c|}{\textbf{M $\Theta_{M,A}$ A $\Theta_{A,D}$ D $\Theta_{D,M}$ M}} \\
        \hline        
        $c_M$ & $c_A$ & $c_D$ & $c_M$\\
        \hline
         \textbf{\textcolor{blue}{M1}} & \textbf{\textcolor{blue}{A60}} & \textbf{\textcolor{blue}{D12}} & \\ 
         \hline
         \textbf{\textcolor{applegreen}{M2}} & \textbf{\textcolor{applegreen}{A2}} & \textbf{\textcolor{applegreen}{D4}} & \textbf{\textcolor{applegreen}{M2}} \\
        \hline
         \textbf{\textcolor{red}{M3}} & \textbf{\textcolor{red}{A36}} & \textbf{\textcolor{red}{D3}} & \textbf{\textcolor{red}{M4}} \\
        \hline
         \textbf{\textcolor{red}{M4}} & \textbf{\textcolor{red}{A1}} & \textbf{\textcolor{red}{D7}} & \textbf{\textcolor{red}{M3}} \\
         \hline
         \textbf{\textcolor{red}{M5}} & \textbf{\textcolor{red}{A276}} & \textbf{\textcolor{red}{D1}} & \textbf{\textcolor{red}{M1}} \\
        \hline
        \end{tabular}
        \label{table:A6-results-allD-itr2}
}
%\qquad
\subfloat[Result]{

    \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{\textbf{\ref{list:We-cyclic3-madm}}, $\omega_e$} \\
 %       \hline
%        \multicolumn{4}{|c|}{\textbf{M $\Theta_{M,A}$ A $\Theta_{A,D}$ D $\Theta_{D,M}$ M}} \\
        \hline        
        $c_M$ & $c_A$ & $c_D$\\
        \hline
         \textbf{\textcolor{blue}{M1}} & \textbf{\textcolor{blue}{A60}} & \textbf{\textcolor{blue}{D12}} \\ 
         \hline
         \textbf{\textcolor{applegreen}{M2}} & \textbf{\textcolor{applegreen}{A2}} & \textbf{\textcolor{applegreen}{D4}} \\
        \hline
         \textbf{\textcolor{blue}{M3}} & \textbf{\textcolor{blue}{A36}} & \textbf{\textcolor{blue}{D3}} \\
        \hline
         \textbf{\textcolor{blue}{M4}} & \textbf{\textcolor{blue}{A1}} & \textbf{\textcolor{blue}{D7}} \\
         \hline
         \textbf{\textcolor{blue}{M5}} & \textbf{\textcolor{blue}{A276}} & \textbf{\textcolor{blue}{D1}} \\
        \hline
        \end{tabular}
        \label{table:A6-results-allD}
}


\caption{Progressive results of a cyclic 3-community}
        \label{table:A6-allD}
    
\end{table}

\end{comment}

%\noindent\textbf{Analysis Results: } After the first iteration of Algorithm \ref{alg:k-community} a 3-community for (A $\Theta_{A,D}$ D $\Theta_{D,M}$ M) will be generated. For the second iteration both the layers ($G_{left} = M$  and $G_{left} = A$) will already have been seen. This iteration will satisfy the case (ii) of the recursive case. As a result of this iteration some pairings will lead to \textit{total matches, cyclic structures} (case ii (a)), some pairings will lead to \textit{inconsistent matches} (case ii (b)) and some communities Movie layer will not be matched to any community in Actor layer leading to \textit{partial matches} (case ii (c)). The inconsistent matches are converted to partial matches by extending the corresponding tuple's second component with an empty bipartite graph (case ii (b)). This analysis shows that the \textbf{even in the absence of total matches, the flexibility of the definition produces some partial matches, that can be used to obtain useful insights}. 
%These cases have been shown in Table \ref{table:A6-results-allD}.


\begin{figure}[h]
   \centering \includegraphics[width=\linewidth]{./figures/A6-madm-v2}
   \caption{Progressive results of a cyclic 3-community}
   %\caption{Cyclic 3-community results for \ref{list:We-cyclic3-madm} with \textcolor{applegreen}{total} and \textcolor{blue}{partial} matches. Inconsistent matches for $\Theta_{D,M}$ shown in \textcolor{red}{red dotted line}}
   \label{fig:A6-madm}
%\vspace{-10pt}
\end{figure}


Results of each successive pairings (there are 3) are shown in Figure~\ref{fig:A6-madm} using the same color notation. Coupling of movie-actor pairs (first composition) results in 5 consistent matches bounded by the movie layer. \textbf{Also, it is easy to see from the figure that only one of them continues and becomes a total element for the cyclic 3-community (\textcolor{blue}{\textbf{bold blue triangle}}.) Further, the final result is an extension (M-A-D-M instead of M-A-D)} \textbf{of the acyclic 3-community result seen in Figure~\ref{fig:A5-mad}.}
When the base case is extended to the director layer (second composition), we got 5 consistent matches %\textbf{only one} matching pair (M2-A2-D4)
as can be seen in Figure~\ref{fig:A5-mad}.  The final composition to complete the cycle uses the 5 communities of director layer and 5 communities of the movie layer as left and right sets of community bipartite graph, respectively. \textbf{Only one consistent match is obtained to generate the total element (M2-A2-D4-M2) for the cyclic 3-community.} It is interesting to see 3 inconsistent matches (\textcolor{red}{red broken lines}) between the communities which clearly \textbf{indicate that all couplings are not satisfied by these pairs.} These result in 3 partial elements (M3-A36-D3, M4-A1-D7 and M5-A276-D1.)

\textbf{The inconsistent matches also highlight the importance of order which is fundamental to our k-community definition for analysis.} If a different order had been chosen (viz. director and actor layer as the base case), the result could have included the inconsistent matches. In this example, we also see \textit{one} no match (\textcolor{blue}{broken blue line}) in the final step, where D12 does not get matched to any movie community, thus generating the partial element, M1-A60-D12.




%%After the first iteration of Algorithm \ref{alg:k-community} a 3-community for (M $\Theta_{M,A}$ A $\Theta_{A,D}$ D) will be generated. For the second iteration both the layers ($G_{left} = D$  and $G_{left} = M$) are already seen. This iteration will satisfy the case (ii) of the recursive case. As a result of this iteration some pairings will lead to \textit{total matches, cyclic structures} (case ii (a)), some pairings will lead to \textit{inconsistent matches} (case ii (b)) and some communities from Director layer will not be matched to any community in Movie layer leading to \textit{partial matches} (case ii (c)). Table \ref{table:A6-results-allD-itr2} highlights the total (marked in \textcolor{applegreen}{green}), partial (marked in \textcolor{blue}{blue}) and inconsistent matches (marked in \textcolor{red}{red}) for this analysis. It is important to note that the inconsistent matches (which mean that the most popular rating for director and actor community are \textit{different}) are also converted to partial matches by extending the corresponding tuple's second component with an empty bipartite graph (case ii (b)). Table \ref{table:A6-results-allD} shows the cyclic 3-community results with the partial results. This analysis shows that the \textbf{even in the absence of total matches, the flexibility of the definition produces some partial matches, that can be used to obtain useful insights}.  




\subsection{Efficiency of Decoupled Approach}
%plot the number of results for A, M, D, A-M, A-D, ..., A-M-D (all sequences), A-M-D (all sequences with cycle)

\begin{figure}[ht]
   \centering \includegraphics[width=\linewidth]{./figures/perf-madm-v1}
   \caption{Performance Results for cyclic 3-community in \ref{list:We-cyclic3-madm}: (M $\Theta_{M,A}$ A $\Theta_{A,D}$ D $\Theta_{D,M}$ M; $\omega_e$)}
   \label{fig:perf-madm}
%\vspace{-10pt}
\end{figure}

The goal of the decoupling approach was to improve the efficiency of k-community detection using the divide and conquer approach. We illustrate that with the largest k-community we have computed which uses 3 iterations (including the base case.)
Figure \ref{fig:perf-madm}(a) shows the execution time for the one-time and iterative costs discussed earlier for \ref{list:We-cyclic3-madm}. The difference in one-time 1-community cost for the 3 layers follow their density shown in Table~\ref{table:layer-stats}. We can also see how the iterative cost is insignificant as compared to the one time cost (by an order of magnitude.) Iteration cost includes creating the bipartite graph, computing $\omega_e$ for meta edges, and maximal flow cost. As the iterations progress, the iterative cost decreases significantly as well. Even \textbf{the cost of all iterations together (0.078 sec) is still almost \textit{an order of magnitude less than the largest one-time cost} (0.694 sec for Movie layer.)} We have used this case as this subsumes all other cases. The zoomed in version (Figure \ref{fig:perf-madm} (b)) of the iterations further show how the iteration cost  reduces. As we had indicated, largest reduction comes for the iteration after the base case which can be clearly seen in Figure~\ref{fig:perf-madm} (b).

%%We believe that the k-community detection can be optimized further. 
The \textbf{additional incremental cost for computing a k-community is extremely small validating the efficiency of decoupled approach}. 
%%Regarding scalability, each layer can be partitioned to compute 1-community. Also, previously computed results can also be leveraged (e.g., weight computation.)

%%%various components involved in progressively generating the cyclic 3-community for \ref{list:We-cyclic3-madm}. It can be seen from Figure \ref{fig:perf-madm} that the one-time (1-community) cost is bound by the densest layer i.e. movie layer. Moreover, as the number of matches are bound by the base case, thus time taken by the last iteration is the least i.e. Time(Base[M-A]) $<$ Time(Iteration-1[A'-D]) $<$ Time(Iteration-2[D'-M']), where A', D' and M' are the respective sets of communities that are part of some tuple in (k-1)-community. Most importantly, \textbf{the total iteration cost (0.078 seconds) is almost order of a magnitude lower than the one-time cost (0.694 seconds for Movie layer)}. Similar observations were made for all other analysis. Thus,  empirically justifying cost efficiency of the proposed decoupled approach of detecting k-community. 


\begin{comment}


\subsection{Insights from k-community Results}

Few interesting insights obtained from the analysis results are as follows

\begin{itemize}
    \item Generally, an actor community will have a majority of the actors belonging to the \textit{same region/country}. On the other hand, any director community groups directors from \textit{around the world based on similar genres}. By pairing up such actor-director communities, one will be able to obtain the groups that are most similar to each other (either directly or by transitive relationship) with respect to \textit{similar movie genres}, \textit{preferred co-actors} and \textit{preferred directors}. Depending on the metric, the same director community can be paired with different actor communities. For example, a person like \textit{Tim Burton} (director of Alice in Wonderland, Planet of the Apes, Dumbo etc.) who belongs to director community 3 that ha directors who primarily make movies from x, y and z genre, is \textit{most similar} to
    \begin{itemize}
        \item co-actor community 1 that has \textit{Indian actors} like Salman Khan (based on \textit{maximum interaction} among actor and director group members - \textbf{Analysis \ref{list:maximum-interaction})},
        \item co-actor community 257 that has \textit{South African actors} like Tim Theron (based on interaction between \textit{strongly connected} actor and director groups - \textbf{Analysis \ref{list:density}}), and
        \item co-actor community 184 with \textit{Egyptian actors} like Lamia El Amir as a member (based on \textit{interaction between most sought after} actors and \textit{versatile} directors - \textbf{Analysis \ref{list:hub-participation})}.
    \end{itemize}
    \item 
    \item 

\end{itemize}

\end{comment}

\begin{comment}


\subsection{Cost of Computation}
\begin{enumerate}
    \item plot of bipartite matching (\textbf{network flow cost}) over iterations. as the number of communities reduce across iterations, BM cost must also reduce
    \item \textbf{layer-wise community detection} is one time cost. can be done in parallel.
    \item for 3 layers, there are 3 complete community bipartite graphs. but 15 sequences possible 2-community (3), 3-community (6 without cycle + 6 with cycle). thus, \textbf{community bipartite graph generation} is also one time cost over different sequences. In general, number of CBGs << number of sequences
    \item Similarly, for each community bipartite graph generated, the three metric values can be calculated with one scan of layer-wise community sets and bipartite graphs that can be used as when required by the analysis. Thus, even \textbf{metric calculation} is one time cost. 
\end{enumerate}

\end{comment}

==> texFiles/old_RelatedWork_1.tex <==
\section{Related Work}
\label{sec:relatedwork}

We present a  summary of the relevant work in the literature with respect to community detection which is the focus of this paper. Community detection has been addressed for various types of graphs - single network (monoplex) and MLNs (homogeneous and hetereogeneous). We indicate how the proposed approach is novel and different from extant approaches. Some background about other related concepts, such as centrality measures and mining are also touched upon.

\noindent \textbf{Single or simple  Network (Monoplex) Analysis:} Plethora of work has been done for detecting communities with an objective to identify groups of vertices that are more connected to each other than to other vertices in the network is often translated into the problem of optimizing network parameters such as modularity ~\cite{clauset2004} or conductance ~\cite{Leskovec08}. The combinatorial optimization problems for community detection are NP-complete ~\cite{Brandes03}. A large number of competitive approximation algorithms exist (see reviews in ~\cite{porter09, Fortunato2009, Xie2013}). Algorithms for community detection have been developed for a wide range of inputs including directed ~\cite{Leicht08,Yang10}, weighted ~\cite{Berry2011}, and dynamic networks ~\cite{Bansal2011,porterchaos13}. Recently there have also been algorithms for identifying overlapping communities~\cite{Yang2013acm,Chakraborty2015a}. Parallel algorithms on different platforms (distributed, shared memory, GPU and MapReduce) have also been implemented ~\cite{StaudtSM14,BhowmickSrinivasan13}.

Other interesting works in monoplexes include i). \textit{finding exact and approximate set of high centrality nodes in graphs} using metrics like degree centrality (vertex degree), closeness centrality (mean distance of the vertex from other vertices), betweenness centrality (fraction of shortest paths passing through the vertex), and eigenvector centrality and its variations, Page Rank and Katz centrality (the number of important neighbors of the vertex)~\cite{Newman2010,ub13,CatalyurekKSS13,GreenB13,FrascaMR12,MadduriEJBC09,Sariyuce2013,SariyuceSKC13,RiedyB13}; ii). \textit{mining interesting patterns in multi-labeled graphs} using substructure discovery~\cite{KDD/HolderCD1994,ICDM/DeshpandeKK2003,ICDM/YanH2002}%,ICDM/KuramochiK2001,Book/InokuchiWT2000}
, apriori approaches - AGM~\cite{VLDB/AgrawalS1994}, FSG~\cite{ICDM/DeshpandeKK2003} or pattern-growth - gSpan~\cite{ICDM/YanH2002}, FFSM~\cite{ICDM/HuanJWWPJ2003} and GASTON~\cite{KDD/NijssenSKJ2004}, disk-based approaches ~\cite{ICDM/PeiHMPCDH2001}, SQL-based approaches ~\cite{dexa/ChakravarthyP08, Dawak/PadmanabhanC09}, and others ~\cite{WWW/SuriV2011,SC/AlamKM13,ilprints1020} and iii). \textit{querying} by converting graphs to indexes - Graph-grep~\cite{pods/ShashaWG02}, G-index~\cite{SIGMOD/YanYH04}, and G-ray~\cite{kdd/TongFGE07} or by query optimization approach~\cite{DaWak/das2016plan}. %However, here we will speak majorly with respect to community detection.


\noindent\textbf{Homogeneous Multilayer Network (HoMLN):} Review of current work on multilayer networks is given in~\cite{MultiLayerSurveyKivelaABGMP13,Boccaletti20141}. Majority of this current work focuses on analyzing homogeneous multilayer networks. These include analysis of co-authorship network in different conferences \cite{MinSubMulLayer2012}, citation network across different topics \cite{ng2011multirank}, interaction network based on calls/bluetooth scans \cite{ClusSpectral2011} and friendship network across different social media platforms \cite{magnani2013formation}. %by considering the layers either \textit{individually or aggregating all of them together}. %Adjacency tensors support \textit{node-aligned networks} and therefore can be used to analyze homogeneous multilayer networks~\cite{de2013mathematical,maruhashi2011multiaspectforensics}.

In terms of \textit{community detection} the work includes algorithms based on matrix factorization \cite{dong2012clustering, qi2012community}, pattern mining \cite{zeng2006coherent,silva2012mining},  cluster expansion philosophy \cite{li2008scalable}, Bayesian probabilistic models \cite{xu2012model} and regression \cite{cai2005mining}. Techniques for determining communities in temporal homogeneous multilayer networks using spectral optimization  of the modularity function based on the supra-adjacency representation have also been proposed \cite{zhang2017modularity,bazzi2016community}. Further, some methods have been developed to determine centrality measures to identify highly influential entities as well \cite{de2013centrality,sole2014centrality,zhan2015influence}. All these techniques \textit{analyze by either aggregating all the layers of the multiplex or by considering the entire multiplex as a whole}. Recently a decoupling-based approach for detecting communities has been proposed to study the combinations of different layers in the network where communities obtained from individual layers are combined to obtain communities in any Boolean operation based combined layer  multilayer network \cite{ICCS/SantraBC17,Arxiv/santra2016scalable}. This technique has also been extended to find highly central nodes for different combinations of layers \cite{ICDMW/SantraBC17}.

\noindent\textbf{Heterogeneous Multilayer Network (HeMLN):} Majority of the work on analyzing heterogeneous multilayer networks (reviewed in \cite{shi2017survey,sun2013mining}) focuses on developing meta-path based techniques for determining the similarity of objects~\cite{sun2011pathsim,he2014exploiting,yao2014pathsimext,wang2016relsim,shi2014hetesim,yu2012user,bu2014integrating,zhang2015top}, classification of objects~\cite{wan2015graph,luo2014hetpathmine,jacob2014learning,wang2016text}, predicting the missing links~\cite{sun2011co,sun2012will,cao2014collective,yu2012citation,chen2013tag,zhang2015organizational}, ranking/co-ranking~\cite{li2014hrank,shi2016constrained,liu2014meta,zhou2007co,zhang2014ncr} and recommendations~\cite{shi2012heterecom,yu2013recommendation,shi2015semantic,yu2014personalized,burke2014hybrid}. An important aspect to be noted here is that most of these work do not consider the intra-layer relationships and concentrate more on the bipartite-type of graph formed by the inter-layer edges while proposing the techniques. %Moreover, we believe most of these operations will benefit from some version of community detection, centrality computation or subgraph mining.
Companies such as Google, Amazon and LinkedIn have built very large  knowledge graphs that connect different types of entities (persons, places, etc.) via multiple edges that describe the relationship through the edge labels. Such graphs can be easily modeled as heterogeneous multilayer networks. However, the analysis of these knowledge graphs is limited to developing search-oriented techniques (\cite{DBLP:conf/cikm/MassS14}, \cite{DBLP:conf/emnlp/GuML15}, \cite{DBLP:conf/www/AbujabalYRW17}). 

In contrast to the homogeneous case, there \textbf{does not exist a consensus on the definition of communities} (and hubs) for heterogeneous multilayer networks. The presence of different sets of entities, inter- and intra-layer edges makes these tasks more challenging. Few existing works have proposed techniques for generating clusters of entities \cite{sun2009rankclus, sun2009ranking,melamed2014community}, but they have only considered the inter-layer links and not the networks themselves. Thus, the combined effect of intra and inter-layer relationships have not been utilized for determining the multilayer communities. In this paper, we will focus on proposing decoupling-based approaches for determining heterogeneous communities.

\begin{comment}
%EARLIER VERSION

We present a short summary of the existing literature on multiplexes and community detection.

\textbf{Heterogeneous Multilayer Networks:}
Majority of the work on analyzing heterogeneous multilayer networks (reviewed in \cite{shi2017survey,sun2013mining}) focuses on developing meta-path based techniques for determining the similarity of objects~\cite{yao2014pathsimext,wang2016relsim}, classification of objects~\cite{wan2015graph,wang2016text}, predicting the missing links~\cite{sun2011co,zhang2015organizational}, ranking/co-ranking~\cite{li2014hrank,shi2016constrained} and recommendations~\cite{shi2012heterecom,shi2015semantic}. An important aspect to be noted here is that most of these work do not consider the intra-layer relationships and concentrate more on the bipartite-type of graph formed by the inter-layer edges while proposing the techniques. Moreover, we believe most of these operations will benefit from some version of community detection, centrality computation or subgraph mining.

Companies such as Google, Amazon and LinkedIn have built very large  knowledge graphs that connect different types of entities (persons, places, etc.) via multiple edges that describe the relationship through the edge labels. Such graphs can be easily modeled as heterogeneous multilayer networks. However, the analysis of these knowledge graphs is limited to search  (\cite{DBLP:conf/cikm/MassS14}, \cite{DBLP:conf/www/AbujabalYRW17}) more than analysis. %Further, the main challenges in achieving high level information fusion \cite{blasch2010high,blasch2012high} is to link information over different collections so that user queries can be answered and patterns can be identified based on information extracted from images, videos, and correlated with other sources to understand frauds, money-laundering, terrorist activities etc. 

%\textbf{Community Detection in Monoplexes:} It involves identifying groups of vertices that are more connected to each other than to other vertices in the network. This objective is often translated into the problem of optimizing network parameters such as modularity ~\cite{Clauset2004} or conductance ~\cite{Leskovec08}. The combinatorial optimization problems for community detection are NP-complete ~\cite{Brandes03}. A large number of competitive approximation algorithms exist (see reviews in ~\cite{porter09, Fortunato2009, Xie2013}). Algorithms for community detection have been developed for a wide range of inputs including directed ~\cite{Leicht08,Yang10}, weighted ~\cite{Berry2011}, and dynamic networks ~\cite{Bansal2011,porterchaos13}.   Recently there have also been algorithms for identifying overlapping communities~\cite{Yang2013acm,Chakraborty2015a}. Parallel algorithms on different platforms (distributed, shared memory, GPU and MapReduce) have also been implemented ~\cite{StaudtSM14,BhowmickSrinivasan13}. %However, only a few of these many algorithms are well known and used by researchers in application domains.

\textbf{Community Detection in Multilayer Networks:} In case of multiplexes, most of the community detection work has been done with respect to the \textbf{homogeneous} variant, that is the one where every layer has the same set of nodes and there are no inter-layer edges. It includes algorithms based on matrix factorization \cite{dong2012clustering, qi2012community}, pattern mining \cite{zeng2006coherent,silva2012mining},  cluster expansion philosophy \cite{li2008scalable}, Bayesian probabilistic models \cite{xu2012model} and regression \cite{cai2005mining}. Techniques for determining communities in temporal homogeneous multilayer networks using spectral optimization  of the modularity function based on the supra-adjacency representation have also been proposed \cite{zhang2017modularity,bazzi2016community}. Moreover, to study the combinations of different layers in the network some efficient approaches have been proposed where communities obtained from individual layers are combined to obtain communities in any Boolean operation based combined layer  multilayer network \cite{ICCS/SantraBC17,Arxiv/santra2016scalable}. %All these techniques analyze by either aggregating all the layers of the multiplex or by considering the entire multiplex as a whole. However, in order to holistically study entities and relationships of multilayer networks, we also have to study the combinations of different layers in the network. Although, techniques based on information theory have been proposed for multilayer protein-protein interactions ~\cite{LayerAggDomenicoNAL14}, this is only for reducing the number of redundant layers through aggregation, but not as a generalized approach for composing different layers that is possible using our proposed network composition approach.
%%Here we propose novel approaches by which communities or central entities obtained from individual layers can be easily combined to obtain communities or central entities present in any composed multilayer network. To the best of our knowledge, this technique of inferring the communities or central entities of the combined network from communities or central entities of individual layers has not been studied before.



%sb Co-communities
However, there \textbf{does not exist a consensus on the definition of communities for heterogeneous multilayer networks}. The presence of different sets of entities, inter- and intra-layer edges makes these tasks more challenging. Few existing works have proposed techniques for generating clusters of entities \cite{sun2009rankclus, sun2009ranking,melamed2014community}, but they have only considered the inter-layer links and not the networks themselves. Thus, the combined effect of intra and inter-layer relationships have not been utilized for determining the multilayer communities. 

\end{comment}

==> texFiles/sc_ProblemStatement.tex <==
\section{Problem Statement}
\label{sec:problem-statement}

%The problem being addressed in this paper can be informally stated as follows. \textit{For a given dataset with M features (explicit or derived) and N entity types along with a set of analysis requirements, i) determine the layers of the homogeneous MLN based on the analysis requirements and ii) develop composition-based community detection algorithms for analysis on arbitrary combinations of layers specified}. Thus, once multiplex layers are created as shown in this paper, any number of analyses can be performed without generating additional graphs/layers. 
We start with a few definitions leading to the formal definition of a community in a MLN.

A graph G = (V, E) is composed of vertices and edges. V is a set of vertices (or nodes) and E $\subseteq$ $V \times V$ is the set of edges of graph G. The size of the graph is defined as the number of vertices of G and it is represented as $|V|$ and the number of edges as $|E|$. If two vertices in G, say \textit{u, v $\in$ V}, are connected by an edge e $\in$ E, this is denoted by \textit{e = (u, v)} and the two vertices are said to be adjacent or neighbors. Edges are said to be undirected when they have no direction. In this paper, all edges are undirected. Note that the above definition does not include multiple edges between nodes, loops, and labels (for both nodes and edges). Our representation and analysis does not require them and we assume unique numbers for nodes across layers.

A multilayer network $MLN (G, X)$, is defined by two sets of single networks. The set $G = \{G_1, G_2, \ldots, G_n\}$ contains general graphs as defined above, where $G_i (V_i, E_i)$ is defined by a set of vertices, $V_i$ and a set of edges, $E_i$. An edge $e(v,u) \in E_i$, connects vertices $v$ and $u$, where $v,u\in V_i$. The set $X =\{X_{1,2}, X_{1,3}, \ldots, X_{n-1,n}\}$ consists of bipartite graphs. Each graph $X_{i,j} (V_i, V_j, L_{i,j})$ is defined by two sets of vertices $V_i$ and $V_j$, and a set of edges (or links) $L_{i,j}$, such that for every link $l(a,b) \in L_{i,j}$,  $a\in V_i$ and $b \in V_j$, where $V_i$ ($V_j$) is the vertex set of graph $G_i$ ($G_j$). 

{\em To summarize}, the set $G$, represents the constituent graphs of layers and the set $X$ represents the graphs that correspond to the edges between a pair of layers. Nodes of X comes from two layers and if labels are assigned, they would have different node labels.

Since we are proposing a decoupling approach for community detection for two layers, we elaborate on our approach below. Figure~\ref{fig:decoupling} shows the approach diagrammatically. Communities for each layer are detected using extant approaches. Layers are then combined pairwise using the bipartite graph approach. Further composition is performed on communities obtained for each layer pair using a join on community identity. The approach is discussed in details in Section~\ref{sec:hemln-community}.

%sc: abhishek, need to slightly modify this fig. drop current approach. show pair-wise composition using bipat approach and join between them.
\begin{wrapfigure}{l}{0.65\textwidth}

   \begin{center}
   \vspace{-30pt}
    \includegraphics[width=0.65\textwidth]{./figures/Decoupling.png}
   \caption{{Current Approach vs Network Decoupling. The difference in pattern in the complete results indicate that the results will be similar, but may not be identical.}}
   \label{fig:decoupling}
\vspace{-10pt}
	\end{center}
\end{wrapfigure}

We define pair-wise network decoupling using two functions (i) $D$, the algorithm for analyzing the constituent networks individually and (ii) $\Theta$, the algorithm for combining the partial results.  Each constituent network, $G_i$, from the heterogeneous multilayer network $N(G,X)$, is analyzed
separately as $D(G_i,X_{i,*})$, where $X_{i,*}$ are the bipartite graphs whose links are connected to $V_i$, to generate the partial results.  The function D is community detection of a single graph corresponding to a layer. The function $\Theta$ is made up og two components: i) the maximum flow algorithm between $G_i$ and any other layer with which  $G_i$ has inter-layer edges and ii) join between communities generated in step i). The paired communities form combined communities between the layers using weights for edges for the bipartite graph based on analysis requirements as discussed in Section~\ref{sec:hemln-community}.

More than two layers are combined using pair-wise communities with a common layer. For example, pair-wise communities for $G_i~and~G_j$ can be joined with pair-wise communities of $G_j~and~G_k$  on community identities of $G_j$. Any number of connected layers can be combined in this way as associativity is satisfied for the join operation.  For a given k layers, the number of pair-wise communities generated as well as the number of join possibilities depends upon the connectivity of layers.

Based on the above, the problem statement can be refined as follows. \textit{For a given dataset with M features (explicit or derived) and N entity types along with a set of analysis requirements,   i) determine the layers of the homogeneous MLN based on the analysis requirements and ii) identify metrics for maximal flow-based bipartite match algorithm and determine the order of joins to form large communities for each analysis.} It is important to note that this formulation of communities preserves entity and feature types as compared to other alternatives proposed in the literature.

Those alternatives are of two kinds: i)  combine (or aggregate) all the layers, ignore types and apply single graph community detection algorithms and ii) projection-based where a layer is projected on to a connected layer as a means of aggregating the two layers and single graph community detection is applied again ignoring entity types.

\sharma{this is a first cut. needs revision and polishing!}

%We express this operation concisely as $D_i$~\footnote{For sake of reducing the number of new terms, we are abusing the notation by representing $D_i$ as both the analysis operation and its corresponding result.}. The partial results are then combined as $D_1 \Theta D_2 \ldots \Theta D_n$. We express this operation concisely as $\Theta_{N}^D$. 


